Poisoning Attacks to Graph-Based Recommender Systems

Recommender system is an important component of many web services to help users locate items that match their interests. Several studies showed that recommender systems are vulnerable to poisoning attacks, in which an attacker injects fake data to a given system such that the system makes recommendations as the attacker desires. However, these poisoning attacks are either agnostic to recommendation algorithms or optimized to recommender systems that are not graph-based. Like association-rule-based and matrix-factorization-based recommender systems, graph-based recommender system is also deployed in practice, e.g., eBay, Huawei App Store. However, how to design optimized poisoning attacks for graph-based recommender systems is still an open problem. In this work, we perform a systematic study on poisoning attacks to graph-based recommender systems. Due to limited resources and to avoid detection, we assume the number of fake users that can be injected into the system is bounded. The key challenge is how to assign rating scores to the fake users such that the target item is recommended to as many normal users as possible. To address the challenge, we formulate the poisoning attacks as an optimization problem, solving which determines the rating scores for the fake users. We also propose techniques to solve the optimization problem. We evaluate our attacks and compare them with existing attacks under white-box (recommendation algorithm and its parameters are known), gray-box (recommendation algorithm is known but its parameters are unknown), and black-box (recommendation algorithm is unknown) settings using two real-world datasets. Our results show that our attack is effective and outperforms existing attacks for graph-based recommender systems. For instance, when 1% fake users are injected, our attack can make a target item recommended to 580 times more normal users in certain scenarios.

==> arXiv - Copy/AttackModel.tex <==
%auto-ignore
\section{Our Poisoning Attacks} \label{AttackModel}
\subsection{Overview}
A solution to the optimization problem in Equation~\ref{objectiveFrame} is a data poisoning attack. 
However, finding the exact optimal solution to the optimization problem in Equation~\ref{objectiveFrame} is computationally intractable (i.e., NP-hard) because 1) the objective function $h(t)$ is related to the rating score variables $r_v$ ($v\in \{v_1,v_2,\cdots, v_m\}$) in a very complex way, and 2) the variables are integer variables. Therefore, we propose techniques to find approximate solutions to the optimization problem. 

%Such integer optimization problems are known to be intractable, and thus finding the optimal solutions can be challenging for an attacker with limited resources. Therefore, we will propose various techniques to solve the optimization problem approximately. 

Specifically, to address the computational challenge, we propose several approximation techniques. First, instead of  optimizing the rating scores for the $m$ fake users simultaneously, we optimize their rating scores one by one. In particular, given the normal users and fake users we have added so far, we find the rating scores for the next fake user to optimize the hit ratio of the target item. Second, we approximate the hit ratio $h(t)$ in the objective function using some function that is easier to optimize. Specifically, since graph-based recommender systems leverage the stationary probabilities of items to make recommendations, our approximate objective function roughly requires that the stationary probabilities of the target item are high for many users. Third, we relax the rating scores to be continuous variables in the range [0, $r_{max}$] and then transform them to integer rating scores after solving the  optimization problem. We propose a projected gradient descent based method to solve the optimization problem with the approximate objective function and relaxed continuous variables.  

%Accordingly, in this section, we shall develop heuristic, a supervised random walk based attack algorithm which relaxes some of the constraints and hence makes the problem tractable. First, instead of solving the intractable integer optimization problem of maximizing $h(t)$, we turn to solve an tractable continuous optimization problem, that is, we want the target items to have a  higher probability to be visited by a large number of users. Then, instead of  rating filler items with integer value while selecting these items, we first use a certain rating strategy to rate items with continuous values, which can also consider as a probability, the probability that a item will be rated by a fake user, after that, we sort all items in descending order by its rating probability and select the top-$n$ ranked items as filler items. After that, we convert the continuous rating probability to discrete integer value by rating each filler item with a integer value drawn from a normal distribution around the mean rating for this item. With this sub-optimal strategy, we could make our optimization problem easier to solve and avoid future detection. Also, while we are solving the continuous optimization problem, we inject fake users one-by-one into the system and ensure that each fake user achieves the optimal attack impact by considering the impact of previously injected fake users. In the last, instead of wanting the target items have a higher probability to be visited by all users, we only consider the target items have a higher probability to be visited by a small set of users, who have the most influence on others' recommendation list. Then our data poisoning attacks algorithm will spoof these users' recommendation list, which indirectly make the target items to be recommended to a large group of users.
%
%Our attack algorithm enjoys low-complexity and more importantly, we show that even using such sub-optimal attacking strategies, our attack can make significant impact with a relatively small attack size, i.e., the ratio between the number of injected fake users and the population of normal users in the system.



\subsection{Approximating the Optimization Problem}
Suppose $t$ is the target item that the attacker aims to promote. We add fake users to the recommender system one by one. Assume $G =  ( U, I, E )$ is the current user preference graph which includes rating scores for both normal users and fake users added so far.  
%We denote by $G =  ( U, I, E )$ a user preference graph and by $t$ the target item that the attacker aims to promote. Assume 
$S$ is the set of normal users who have not rated the target item $t$. We denote the set of top-$N$ recommended items for a user $u$ as ${L_u}$.

\myparatight{Relaxing rating scores to be continuous variables} We add a fake user $v$ to the user preference graph $G$, where $w_{vi}$ is the rating score that the fake user gives to item $i$. We model $w_{vi}$ as the weight of the edge $(v,i)$. For simplicity, we denote by $w_v$ the vector of weights of edges that connect the fake user $v$ and all items. 
Our goal is to find the edge weights $w_v$ that optimize the hit ratio of the target item.  Since rating scores are integers, $w_v$ are integer variables whose values could be $0,1,\cdots, r_{max}$. However, such integer variables make the optimization problem intractable. Therefore, we  relax the variables  as continuous variables whose values are in the range [0, $r_{max}$], solve the optimization problem using the continuous variables, and transform them to integer rating scores. Note that $w_{vi}$ is different from $r_{vi}$. Specifically, $w_{vi}$ is a continuous variable we use to model a rating score, while $r_{vi}$ is the final integer rating score that user $v$ gives to item $i$. 

\myparatight{Approximating the hit ratio} Since the hit ratio is related to the edge weights $w_v$ in a very complex way, which makes the optimization problem intractable, we approximate the hit ratio using the stationary probabilities of random walks, which are used to generate the top-$N$ recommended items in graph-based recommender systems. 
 In the user preference graph with the new fake user $v$, to make recommendations for a normal user $u$, we first perform a random walk from $u$ and compute its stationary probability distribution $p_u$, where $p_{ui}$ is the stationary probability for item $i$. Specifically, the stationary probability distribution $p_u$ is computed according to Equation~\ref{RWR}, where the transition matrix $Q$ is a function of the edge weights $w_v$. The recommendation list $L_u$ consists of the $N$ items that 1) $u$ has not rated yet and 2) have the largest stationary probabilities. The target item $t$ hits the user $u$ if $t$ is among the recommendation list $L_u$, i.e., if $p_{ut}> p_{ui}$ for a certain item $i$ in the recommendation list $L_u$, otherwise the target item does not hit the user $u$.

{\bf 1) Loss function for one user.} To approximate the hit ratio, we leverage a \emph{loss function} $l_u$ over the stationary probability distribution for each user $u$. We aim to design a loss function that satisfies two goals: 1) for each item $i\in L_u$, if $p_{ui} < p_{ut}$ (i.e., the target item ranks before the item $i$), then the loss for item $i$ is smaller,  and 2) the loss is smaller if the target item ranks higher in the recommendation list $L_u$. To achieve these goals, we adopt the following loss function:
\begin{align}
l_u=\sum_{i \in L_u} g(p_{ui} - p_{ut}),
\end{align} 
where $g(x) = \frac{1}{{1 + \exp (-{x/b})}}$ is called the Wilcoxon-Mann-Whitney loss function~\cite{backstrom2011supervised} and $b$ is a parameter called \emph{width}. In the machine learning community, the Wilcoxon-Mann-Whitney loss function is known to optimize the ranking performance~\cite{backstrom2011supervised}, i.e., the loss is smaller when the target item ranks higher in the recommendation list in our case. 

{\bf 2) Loss function for all normal users.} Our goal is to recommend the target item to as many normal users as possible. Therefore, we sum the loss of all normal users as follows:
\begin{align}
l=\sum_{u \in S} l_u,
\end{align}
where $S$ is the set of normal users who have not rated the target item yet. 


{\bf 3) Approximate optimization problem.} Recall that, in our threat model, each fake user rates at most $n$ items to avoid detection, which essentially constrains the values of $w_v$. Considering this constraint, we propose to solve the following optimization problem:
\begin{align}
\min F(w_v) &= {\left\| w_v \right\|_2^2} + \lambda \cdot l \nonumber\\
\label{appproblem}
\text{subject to } &w_{vi} \in [0, r_{max}],
\end{align}
where $\left\| w_v \right\|_2^2$ regularizes $w_v$ and is used to model the constraint that each fake user can rate a small number of items, while $\lambda$ balances the regularization term and the loss function. 


%The loss function has a smaller value when the target item is ranked higher in the recommendation list $L_u$. Specifically, for each item $i\in L_u$, we define a loss $h(p_{ui}-p_{ut})$, where if $p_{ui}-p_{ut} >0$, then the loss 
%
%
%Given $m$ fake users to be injected, our algorithm injects one fake user at a time. When the $i$-th fake user $v_i$ is to be injected, we want to maximize its impact on promoting the target item $t$. To make it easy to follow, we first consider how to promote $t$ to a single normal user $s \in S$. Specifically, \textit{for any random walk path originating from $s$, we want the injection of $v_i$ to cause the walk path to become more likely to visit $t$}. Recall that the items that are most likely to appear on the path originate from $s$ are used as candidates for its top-$N$ recommendation list, hence such a path will increase the probability that $t$ will be recommended to $s$ as the attacker desires.
%
%A random walk path from $s$ is calculated as follows: We start by setting the current node $u$ to $s$. Then, we randomly select a node that is connected to $u$ as the next node on the path. The probability that a node $v$ being selected is set to be proportion with the weight on edge $(u, v)$. After that, the next node is updated as current node, and this process is repeated until a maximal path length is reached. In order to influence the random walk path, the algorithm needs to carefully select a set of filler items to be rated by the fake user ${v_i}$. The filler items will serve as intermediate nodes on the random walk path from the user $s$ to the item $t$, and hence can increase the probability that $t$ appears on the path. To maximize the chance that $t$ will be recommend to $s$, we want to achieve $p_t > p_i, \forall  i \in {L_s^N}$, where $p_i$ is the probability that $i$ appears on the random walk path from $s$. That is, we want target item $t$ to have the highest probability to appear on the random walk path from $s$ comparing with any other item in ${L_s^N}$.
%
%Figure~\ref{attack-idea} illustrates the general idea of our proposed attack with a set of 3 users and 5 items. Suppose our goal is to recommend item $i_2$ to user $u_1$, whose recommendation list includes two items $L_{{u_1}}^N = \{ {i_4},{i_5}\}$, but not $i_2$. Our attack injects a fake user $v$, who gives positive rating to three items: the target item $i_2$ and the two filler items ${I_F}({v}) = \{ {i_3},{i_4}\}$. The filler items are selected to ensure $p_{i_2} > p_i, \forall  i \in {L_{{u_1}}^N}$. Hence, the probability that $i_2$ will be recommend to $u_1$ is maximized by our attack.
%
%\begin{figure}[!t]
%	\centering
%	\includegraphics[scale = 0.45]{figs/fig2.pdf}
%	\caption{An example of the proposed attack method.}\label{attack-idea}
%\end{figure}
%
%We now consider how to generalize this idea to promote $t$ to as many as possible normal users in $S$. The objective value we want to maximize is the expectation of the number of users in $S$ to whom $t$ will be recommended to after the attack. That is, when a fake user $v_i$ is injected, our goal is to maximize its impact on the random walk path from not only one user $s$, but as many as possible normal users. To achieve the desired impact, it is also necessary to take into account the impacts from fake users $\{v_1, v_2, ... v_{i-1} \}$ which are injected in the previous $i-1$ steps. 
%
%Let ${w_{{v_i}}}(j)$ denote the probability that we select item $j$ as a filler item for fake user ${v_i}$, where $0 \le {w_{{v_i}}}(j) \le 1$. We also assume filler items are selected from a candidate item set, denoted by $C$, where $C \triangleq I\backslash \{ t\}$. We want to find a set of parameter values $w = \{ {w_{{v_i}}}(j), 1 \leq i \leq m, j \in C \}$ which will maximize our objective value. $w$ can be found by solving the following optimization problem:
%\begin{align}
%\mathop {\min {\kern 1pt} }\limits_w {\kern 1pt} F(w) = {\left\| w \right\|^2} + \lambda \sum\limits_{s \in S} {\sum\limits_{x \in L_s^N} {h({p_x} - {p_t})}},
%\end{align}
%where $p$ is the stationary distribution of random walk, $\lambda$ is the regularization term used to avoid overfitting the parameters, and $h( \cdot )$ is a non-negative loss function. Note that it is very likely that there does not exist a set of parameter values that guarantees $p_t > p_i, \forall  i \in {L_s^N}$ for all the users in $S$. Thus the loss function is in place to measure the penalty of not achieving this optimal goal. If ${p_x} - {p_t} > 0$ then $h( \cdot ) > 0$, if ${p_x} - {p_t} < 0$ then $h( \cdot ) = 0$. Here we choose the commonly-used Wilcoxon-Mann-Whitney loss function as recommended in~\cite{backstrom2011supervised},
%\begin{align}
%h(x) = \frac{1}{{1 + \exp ( - {x \mathord{\left/  {\vphantom {x b}} \right.  \kern-\nulldelimiterspace} b})}},
%\end{align}
%where $b$ is the width. The rating between fake user and each item is calculated with an \textit{edge strength function}, for which we use the logistic function:
%\begin{align}
%{f(w)} = \frac{1}{{1 + \exp ( - w)}}.
%\end{align}
%
%Nonetheless, solving the above optimization problem can still be challenging due to the large search space. Since modern recommender systems usually involve millions of users, finding the global optimal solution can be extremely expensive in reality.
%
%We are interested in finding an attack algorithm that can significantly reduce this cost without having to scarify too much performance. To this end, our method is to consider only a small subset of users in the optimization problem who have the most influence on others recommendation lists. We call such users as the \textit{top-$k$ most positive users}. In order to define the most positive users, we first introduce the concept of \textit{average rating} $\overline {{r_u}}$ of a user $u$：
%\begin{align}
%\label{averageRating}
%\overline {{r_u}}  = \frac{{\sum\limits_{i \in {I_u}} {{r_{ui}}} }}{{\left| {{I_u}} \right|}},
%\end{align}
%where ${{I_u}}$ is the set of items which user $u$ has rated, ${\left| {{I_u}} \right|}$ is the number of items in ${{I_u}}$. Formally, we define top-$k$ most-positive users as follows:
%\begin{definition}
%We say $k$ users who has the highest value of average ratings for items are the \textbf{Top-$k$ Most-Positive Users}.
%\end{definition}
%Intuitively, most positive users are those with most positive average ratings, since many companies want to avoid bad ratings for their products, it is a ``safe'' strategy to focus on these users. In the preference graph, most positive users are more likely to be one a random walk path due to the fact that their corresponding nodes have higher degree. Hence, the preference of these users can have high impact on many other users' recommendation list. Our key hypothesis is that, by manipulating the recommendation list of these most positive users, we can achieve the goal of promoting the target item to a large number of normal users:
%
%\begin{hypothesis}
%Making the target item $t$ to appear in the recommendation list of top-$k$ most positive users will result in $t$ being recommended to a large number of users in $S$.
%\end{hypothesis}
%
%Based on the above hypothesis, we design an attack algorithm that focuses on leveraging the top-$k$ most positive users. In our algorithm, we only consider top-$k$ positive users who have not rated the target item $t$. Let $\kappa$ denote the set of top-$k$ most positive users. Our algorithm solves the following optimization problems, which has a much smaller searching space:
%\begin{align}
%\label{rwrOPt}
%\mathop {\min {\kern 1pt} }\limits_w {\kern 1pt} F(w) = {\left\| w \right\|^2} + \lambda \sum\limits_{s \in \kappa} {\sum\limits_{x \in L_s^N} {h({p_x} - {p_t})} }.
%\end{align}


\begin{algorithm}[!t]
	\caption{\textit{Our Poisoning Attacks}}\label{attack_algo}
	\begin{algorithmic}[1]
		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		\renewcommand{\algorithmicensure}{\textbf{Output:}}
		\REQUIRE  Rating matrix $R$, parameters $t, m, n, \lambda, b$.
		\ENSURE  $m$ fake users $v_1, v_2, \cdots, v_m$.
%		\STATE Initialization: ${R_t} = R$.
%		\STATE Select Most-Positive Users set $\kappa$ according to Equation~(\ref{averageRating}).
		\STATE //Add fake users one by one.
		\FOR {$ v = v_1, v_2, \cdots, v_m$}
%			\STATE $w \leftarrow w_0$.  
%			\FOR{each $s \in \kappa$}
%				\STATE Run random walk from $s$ and get its top-$N$ recommendation list as ${L_s^N}$. 
%			\ENDFOR
			\STATE Solve the optimization problem in Equation \ref{appproblem} with the current rating matrix $R$ to get $w_v$.			
%			 $\frac{{\partial F(w)}}{{\partial w}}$ according to Equation~(\ref{rwrOPtMIN}).
			\STATE //Assign the maximum rating score to the target item.
			\STATE $r_{vt} =  r_{max}$.
			\STATE //Find the filler items
			\STATE The $n$ items with the largest weights are filler items.
			\STATE //Generate rating scores for the filler items.
			\STATE  $r_{vj} \sim \mathcal{N}(\mu_{j},\,\sigma_{j}^{2})$, for each filler item $j$. 
			\label{normaldistribution}
			\STATE //Inject the fake user with rating scores $r_v$ to the system.
			\STATE $R\leftarrow R \cup r_v$.  
		\ENDFOR
		\RETURN $r_{v_1}, r_{v_2}, \cdots, r_{v_m}$. 
	\end{algorithmic} 
\end{algorithm}


\subsection{Solving the Optimization Problem}
We solve the optimization problem in Equation~\ref{appproblem} using \emph{projected gradient descent}. Specifically, in each iteration, we compute the gradient of $F(w_v)$ with respect to $w_v$, move $w_v$ a small step towards the inverse direction of the gradient, and project each $w_{vi}$ back to the range $[0,r_{max}]$. We can compute the gradient of $F(w_v)$ as follows: 
\begin{align}
\label{rwrOPtMIN}
\begin{split}
\frac{{\partial F(w_v)}}{{\partial w_v}} &= 2w_v + \lambda \sum_{u \in S} {\sum_{i \in L_u} {\frac{{\partial g(p_{ui} - p_{ut})}}{{\partial w_v}}}} \\
&= 2w_v + \lambda \sum_{u \in S} {\sum_{i \in L_u} {\frac{{\partial g({\delta _{it}})}}{{\partial {\delta _{it}}}}} } (\frac{{\partial p_{ui}}}{{\partial w_v}} - \frac{{\partial {p_{ut}}}}{{\partial w_v}}),
\end{split}
\end{align}
where ${\delta _{it}} = p_{ui} - p_{ut}$. 

The key challenge of computing the gradient is to compute the gradient $\frac{{\partial {p_u}}}{{\partial w_v}}$ for each normal user $u$.
 From Equation~\ref{RWR}, we have:
%To solve this optimization problem, we derive the gradient of $F(w)$ with respect to $w$, and gradient based optimization methods (e.g., steepest descent or L-BFGS) can be used to solve the following problem:
%\begin{align}
%\label{rwrOPtMIN}
%\begin{split}
%\frac{{\partial F(w)}}{{\partial w}} &= 2w + \lambda \sum\limits_{s \in \kappa} {\sum\limits_{x \in L_s^N} {\frac{{\partial h({p_x} - {p_t})}}{{\partial w}}}} \\
%&= 2w + \lambda \sum\limits_{s \in \kappa} {\sum\limits_{x \in L_s^N} {\frac{{\partial h({\delta _{xt}})}}{{\partial {\delta _{xt}}}}} } (\frac{{\partial {p_x}}}{{\partial w}} - \frac{{\partial {p_t}}}{{\partial w}}),
%\end{split}
%\end{align}
%where ${\delta _{xt}} = p_x - p_t$. To find partial derivatives of $\frac{{\partial {p_u}}}{{\partial w}}$, from Equation~(\ref{RWR}) we have:
\begin{align}
\label{p_to_w}
\frac{{\partial {p_u}}}{{\partial w_v}} = (1 - \alpha )\frac{{\partial Q}}{{\partial w_v}}{p_u} + (1 - \alpha )Q\frac{{\partial {p_u}}}{{\partial w_v}}.
\end{align}

Furthermore, according to Equation~\ref{matrixQ}, we have: 
%To obtain $\frac{{\partial Q}}{{\partial w}}$, from Equation~(\ref{matrixQ}), when $(x, y) \in E$, we have:
\begin{align}
\label{Q_to_w}
\frac{{\partial {Q_{xy}}}}{{\partial w_v}} = 
\begin{cases}
\frac{{\frac{{\partial {w_{xy}}}}{{\partial w_v}}\sum\nolimits_j {{w_{xj}} - {w_{xy}}\sum\nolimits_j {\frac{{\partial {w_{xj}}}}{{\partial w_v}}} } }}{{{{(\sum\nolimits_j {{w_{xj}}} )}^2}}}, \text{ if } (x, y) \in E \\
0, \text{ otherwise,}
\end{cases}
\end{align}
where $w_{xy}$ is the discrete rating score that user $x$ gave to the item $y$ when $x$ is not the new fake user, and $w_{xy}$ is the continuous edge weight to be optimized when $x$ is the new fake user. 
Therefore, Equation~\ref{p_to_w} is a linear system of equations with respect to $\frac{{\partial {p_u}}}{{\partial w_v}}$. We iteratively solve the linear system to obtain $\frac{{\partial {p_u}}}{{\partial w_v}}$. After solving $\frac{{\partial {p_u}}}{{\partial w_v}}$, we can compute the gradient 
$\frac{{\partial F(w_v)}}{{\partial w_v}}$.

%By recursively applying the chain rule to Equation~(\ref{p_to_w}) and Equation~(\ref{Q_to_w}), $\frac{{\partial {p_u}}}{{\partial w}}$ can be iteratively computed by converging to a defined threshold.


%To solve this optimization problem, we follow the same steps in ~\cite{backstrom2011supervised}. We first derive the gradient of $F(w)$ with respect to $w$, and then use gradient-based method (e.g., steepest descent or L-BFGS) to find $w$ that minimize $F(w)$. The pesudocode shown in Algorithm~\ref{attack_algo} describes the concrete steps of the complete data poisoning attacks algorithm.





\subsection{Generating Rating Scores}
After solving the weights $w_v$, we generate rating scores for the fake user $v$. First, we assume the fake user gives the maximum rating score to the target item. Second, we rank the items according to the weights $w_{vi}$ and select the $n$ items with the highest weights as the filler items. The fake user only generates rating scores for the filler items. Third, for each filler item, we sample a number  from a normal distribution that is fitted to the rating scores that all normal users gave to the item, and then discretize the number to an integer rating score. We only use the weights to select filler items instead of assigning their rating scores, because the weights are approximate values. We generate rating scores for the filler items from such a normal distribution so that the fake user is  likely to be similar to more normal users, which makes it more likely to recommend the target item to more normal users. 

Algorithm~\ref{attack_algo} summarizes our poisoning attacks. We generate fake users one by one. For each fake user, we use projected gradient descent to solve the optimization problem in Equation~\ref{appproblem} with the current rating score matrix (i.e., the current user preference graph). After solving the weights $w_v$, we generate rating scores. Specifically, $\mathcal{N}(\mu_{j},\,\sigma_{j}^{2})$ at Line~\ref{normaldistribution} is the normal distribution with mean $\mu_{j}$ and variance $\sigma_{j}^{2}$ that are fitted using the rating scores that normal users gave to the item $j$.

% to The algorithm runs in phases (Lines 1-13). After using Equation~(\ref{averageRating}) to get top-$k$ most positive users (Line 2), the algorithm injects one fake user into system in each iteration to ensure each fake user achieves the optimal attack impact (Lines 3-12). For each fake user, our algorithm first initializes $w$ with a initial value $w_0$ (Line 4), then it performs a random walk from each positive user $s$ to get its corresponding top-$N$ recommendation list ${L_s^N}$ (Lines 5-7). After we use gradient-based method to find the optimal solution $w$ of Equation~(\ref{rwrOPtMIN}) (Line 8), we sort $w$ in descending order and select the top-$n$ ranked items as filler items (Line 9). In Line 9, we only select the filler items, but do not rate items with the rating of $w$ computed according to Equation~(\ref{rwrOPtMIN}). Because a fake user may rate most of {\tiny }its filler items with the same rating when normalize $w$ to an integer value, and this could easily be detected by the system. Therefore, in Line 10, we rate the target item $t$ with the maximum rating value, and rate each item $j \in {I_F}({v_i})$ with a integer value draw from a normal distribution around the mean rating for $j$, where $\mu_{j}$ and $\sigma_{j}^{2}$ are mean and variance of ratings for item $j$ across all normal users. The intuition is that, we want to mimic normal user behaviors to avoid potential detection since normal users generally do not rate items at random. Subsequently, we inject the attack profile of fake user $v_i$ into the system and update the rating matrix $R_t$. 

%After we use gradient-based method to find the optimal solution $w$ of Equation~(\ref{rwrOPtMIN}) (Line 8), we sort $w$ in descending order and select the top-$n$ ranked items as filler items (Line 9). In Line 9, we only select the filler items, but do not rate items with the rating of $w$ computed according to Equation~(\ref{rwrOPtMIN}). Because a fake user may rate most of {\tiny }its filler items with the same rating when normalize $w$ to an integer value, and this could easily be detected by the system. Therefore, in Line 10, we rate the target item $t$ with the maximum rating value, and rate each item $j \in {I_F}({v_i})$ with a integer value draw from a normal distribution around the mean rating for $j$, where $\mu_{j}$ and $\sigma_{j}^{2}$ are mean and variance of ratings for item $j$ across all normal users. The intuition is that, we want to mimic normal user behaviors to avoid potential detection since normal users generally do not rate items at random. Subsequently, we inject the attack profile of fake user $v_i$ into the system and update the rating matrix $R_t$. 





==> arXiv - Copy/conclusion.tex <==
%auto-ignore
\section{Conclusion and Future Work} \label{sec:conclusion}

In this work, we propose optimized poisoning attacks to graph-based recommender systems. We show that poisoning attacks to graph-based recommender systems can be formulated as an optimization problem and the optimization problem can be approximately solved by a projected gradient descent method. Via evaluations on real-world datasets, we find that our attacks can make a target item recommended to substantially more users. Moreover, our attacks are more effective than existing attacks for manipulating graph-based recommender systems. The reason is that existing attacks are not optimized for graph-based recommender systems, while our attacks are. Our attacks can also transfer to other recommender systems under the gray-box and black-box settings. The service provider can detect a large fraction of fake users but also falsely predict a small fraction of normal users to be fake, via using supervised machine learning techniques to analyze the users' rating scores. Moreover, our attacks are still effective when the service provider deploys such a detector and excludes the predicted fake users from the recommender system. %The reason is that a large fraction of fake users are not detected and some normal users are falsely detected. 

Interesting future works include 1) evaluating our poisoning attacks on real-world graph-based recommender systems, 2) designing optimized poisoning attacks to other graph-based recommender systems (e.g., graph convolutional neural network based recommender systems~\cite{Ying18}), 3) designing optimized poisoning attacks to neural network based recommender systems (e.g.,~\cite{He17}), and 4) designing defenses against poisoning attacks.



\section*{Acknowledgements}
We thank the anonymous reviewers for their insightful feedback. This work is supported by the National Science Foundation under Grants No.
 CNS-1750198 and CNS-1801584. Any opinions, findings and conclusions or recommendations
expressed in this material are those of the author(s) and do
not necessarily reflect the views of the funding agencies.

==> arXiv - Copy/experiments.tex <==
%auto-ignore
\section{Experiments} \label{sec:exp}


\begin{table}[!t]
\centering
\caption{Dataset statistics.}\label{datasets}
\begin{tabular}{ccccc} 
\hline
Dataset &\#Users  &\#Items  &\#Ratings  &Sparsity\\ \hline  
Movie &943 &1,682 &100,000 &93.67\% \\     
Video &5,073 &10,843 &48,843 &99.91\%\\ \hline
\end{tabular}
\end{table}


%\subsection{Recommendation Algorithms (RAs)}
%
%We implement a graph-based recommender system, namely Random Walk with Restart (RWR), as the target of our attack. Although our algorithm is developed with a focus on graph-based recommender systems, we also implement a Matrix Factorization-based recommender systems and test the proposed attack on these systems. These two algorithms are widely used by recommender systems.
%
%\textbf{Random Walk with Restart (RWR)} RWR~\cite{tong2006fast} performs a random walk on the user preference graph $G =  ( U, I, E )$. The random walk path follows the edges with a certain probability that resembles the transition probability from one node to another. This transition is biased by the edge weight. Consequently, we can define the transition matrix $Q$ as:
%\begin{align}
%{Q_{ui}} = \begin{cases}
%\frac{{{r_{ui}}}}{{\sum\limits_{j \in {I_u}} {{r_{uj}}} }}, & \mbox{if $(u, i) \in E$},\\
%0, & \mbox{otherwise}.
%\end{cases}
%\end{align}
%The intuition behind RWR is that the higher the rating score ${{r_{ui}}}$ is, the higher is the transition probability. Furthermore, RWR assigns a restart probability $\alpha$ for the random walk, i.e., the probability the random walk path will jump back to the start node $s$, and thus the final stationary distribution $p$ will be:
%\begin{align}
%\label{RWR1}
%p = (1 - \alpha ) \cdot Q \cdot p + \alpha  \cdot e_s,
%\end{align}
%where $e_s$ is a unit vector satisfying $e_s(s) = 1$ and all other values are set to 0. RWR algorithm iteratively applies Equation~(\ref{RWR}) until it converges. It then uses the stationary distribution $p$ to rank the nodes (items) and make recommendations with the top-$N$ items. Specifically, the top-$N$ items are recommended to user $u$ if they do not belong to user's rating item set ${{I_u}}$.
%
%\textbf{Matrix Factorization (MF):} Matrix factorization~\cite{MFRec09} is one of the most popular recommendation algorithms. MF maps users and items into a latent factor of $d$-dimensional space, user $u$ is represented by a latent vector $x_u \in {{\mathbb{R}}^{d}}$ and item $i$ by a latent factor $y_i \in {{\mathbb{R}}^{d}}$. A rating predicted by user $u$ to item $i$ is given by
%\begin{align}
%\hat{r}_{ui} = \mu  + {b_i} + {b_u} + y_i^T{x_u},
%\end{align}
%where $\mu$ is the total average of all ratings, $b_u$ and $b_i$ are the user and item biases respectively. We can learn the parameters ($b_u$, $b_i$, $x_u$ and $y_i$) by minimizing the following objective function:
%\begin{align}
%\mathop {\min }\limits_{{x^*},{y^*},{b^*}} {\sum\limits_{u,i} {({r_{ui}} -\hat{r}_{ui})} ^2} + \eta (||{x_u}|{|^2} + ||{y_i}|{|^2} + ||{b_u}|{|^2} + ||{b_i}|{|^2}),
%\end{align}
%where $\eta$ is the regularization parameter. Although MF is effective in making good recommendations, it is also known to suffer from the cold start problem~\cite{MFRec09}, i.e., it is challenging to generate high-quality recommendations for users who have little item rating/visiting history.



\subsection{Experimental Setup}

\subsubsection{Datasets}
We perform experiments using two real-world datasets, which are widely used for evaluating recommender systems in the data mining community. The first dataset is \textbf{MovieLens 100K (Movie)}~\cite{movielensURL}. This dataset consists of 943 users, 1,682 movies, and 100,000 ratings. 
%The sparsity of Movie is 93.67\%. 
The second dataset is \textbf{Amazon Instant Video (Video)}~\cite{amazonURL}, which includes 5,073 users, 10,843 items, and 48,843 ratings. %The original dataset contains 400k users, 20k instant videos and 500k ratings. For our experiments, we discard the users who have rated less than 6 instant videos. This resulted in 5,073 users, 10,843 items and 48,843 ratings.
We define the \textit{sparsity} of a dataset as follows:
\begin{align}
Sparsity = 1 - \frac{\text{number of ratings}}{\text{number of users} \times \text{number of items}}.
\end{align}
As we will show, the attack performance is related to the sparsity of a recommender system.  Table~\ref{datasets} shows the dataset statistics. 

%where $N_r$ is the total number of user ratings included in the dataset. The first dataset we used is \textbf{MovieLens 100K (Movie)}. This dataset consists of 943 users, 1,682 movies and 100,000 ratings. The sparsity of Movie is 93.67\%. The second dataset we use is \textbf{Amazon Instant Video (Video)}. The original dataset contains 400k users, 20k instant videos and 500k ratings. For our experiments, we discard the users who have rated less than 6 instant videos. This resulted in 5,073 users, 10,843 items and 48,843 ratings. The sparsity of this dataset is 99.91\%. (Table~\ref{datasets})

\subsubsection{Compared Attacks} We compare our poisoning attacks to several poisoning attacks. In all these attacks, an attacker injects $m$ fake users to the recommender system. Each fake user gives the maximum rating score to the target item and gives certain rating scores to $n$ selected items (called \emph{filler} items). Different attacks use different strategies to select the filler items and generate rating scores for them. 

\myparatight{Random attack~\cite{lam2004shilling}} In this attack, the attacker first fits a normal distribution for the rating scores in the entire user-item rating score matrix.  For each fake user, the attacker selects $n$ items as the filler items uniformly at random. Then, for each filler item, the attacker samples a number from the normal distribution and discretizes it to be a rating score. 

%Random attack is a naive attack. In this attack model, the attacker creates profiles by selecting filler items randomly, and rates each filler item with a normal distribution around the mean rating value across the whole database. Then the maximum rating value for the target item is added to the newly created profile.

\myparatight{Average attack~\cite{lam2004shilling}} In this attack, the attacker fits a normal distribution for the rating scores of each item. Like the random attack, average attack also samples $n$ items as filler items uniformly at random. However, for each filler item, the attacker generates a rating score from the normal distribution fitted for the item. The intuition is that generating rating scores around the average rating scores of filler items could enable the fake users to be more similar to normal users, and thus have a larger effect on the recommendations.


%Average attack is more sophisticated than random attack in the sense that it takes advantage of the knowledge of the average rating of each item in the recommender system. In this attack, attacker also select filler items randomly, but rate each filler item with a normal distribution around the mean rating for this item. The rational behind this attack is that providing rating around the average rating of each filler item will help the attacker be more similar to normal users, thus, having a larger effect on the recommendations. As with the random attack, the target item is rated with the maximum rating value.

\myparatight{Bandwagon attack~\cite{mobasher2007toward}} This attack considers item popularity when selecting filler items. We implement a variant of bandwagon attack as follows: for each fake user, the attacker selects $n\times 10\%$ items whose average rating scores are high (e.g., 5 in our experiments) and selects $n\times 90\%$ items uniformly at random as filler items. For each filler item, the attacker generates a rating score from the normal distribution fitted for the entire user-item rating score matrix (like the random attack). The intuition is that the attacker aims to recommend the target item to users who rated the popular items. 

%advanced attack model leverages Zipf's law distribution of popularity and then generates the biased profiles that contain frequently rated items~\cite{mobasher2007toward}. Here, filler items is a set of most frequently rated items. The rating value for each filler item is drawn from a normal distribution around the mean rating value across the whole dataset. Similar to random and average attack, the maximum rating value is assigned to the target item.



\myparatight{Co-visitation attack~\cite{yang2017fake}} This attack was designed for association-rule-based recommender systems. We note that in the original attack, the attacker does not necessarily need to register fake users, because some association-rule-based recommender systems consider visitations from any visitors to make recommendations. In our work, we focus on recommender systems using rating scores and only registered users can provide rating scores. Therefore, the attacker injects fake users to the system. Moreover, if a user rates both items $i$ and $j$, then we say $i$ and $j$ are co-visited by the user. Therefore, the attack technique developed by Yang et al.~\cite{yang2017fake} essentially finds the filler items for each fake user. For each filler item of each fake user, we generate a rating score from the normal distribution fitted for the item (like the average attack). 

%user-item matrix rating This attack is performed by injecting fake co-visitations between a target item and carefully selected filler items. The attack goal can be prompting or demoting a selected item. We allow each fake user to inject $n$ fake co-visitations in this attack.

\subsubsection{Target Items (Random Target Items vs. Unpopular Target Items)} We consider two types of target items. First, an attacker aims to promote a \emph{random} target item.  Specifically, in our experiments, we sample an item uniformly at random and treat it as the target item. Second, an attacker could also promote an unpopular item (e.g., a new item that belongs to the attacker). To simulate this attacker, we sample an item that has 5 ratings at most uniformly at random and treat it as the target item. 
%number of ratings is no larger than 5 uniformly 


\subsubsection{Evaluation Metric (HR@N)} We use the hit ratio (HR@N) as our evaluation metric. Suppose the recommender system recommends $N$ items for each user. Given a target item, HR@N is the fraction of normal users whose $N$ recommended items include the target item. For both random target items and unpopular target items, we compute the hit ratio averaged over 10 target items. 

% and design four tasks to evaluate the performance of our proposed data poisoning attacks, which are described below.

\subsubsection{Parameter Setting} Without otherwise mentioned, we use the following \emph{default parameter setting}: the restart probability $\alpha$ in graph-based recommender systems is set to be 0.3, $\lambda = 0.01, b = 0.01, N = 10$, and $n=10$. Moreover, the number of fake users (i.e., \emph{attack size}) is 3\% of the normal users in the recommender system. By default, we assume graph-based recommender system is used. %The default recommender system in this paper is RWR. The default attack targets in our experiments are the same as data poisoning attacks.



%\subsection{Results}


%\subsection{Baselines}
%For a comprehensive performance evaluation, we use three typical attacks discussed in~\cite{mobasher2007toward} and co-visitation attack~\cite{yang2017fake} as baselines.
%
%\textbf{Random Attack:} Random attack is a naive attack. In this attack model, the attacker creates profiles by selecting filler items randomly, and rates each filler item with a normal distribution around the mean rating value across the whole database. Then the maximum rating value for the target item is added to the newly created profile.
%
%\textbf{Average Attack:} Average attack is more sophisticated than random attack in the sense that it takes advantage of the knowledge of the average rating of each item in the recommender system. In this attack, attacker also select filler items randomly, but rate each filler item with a normal distribution around the mean rating for this item. The rational behind this attack is that providing rating around the average rating of each filler item will help the attacker be more similar to normal users, thus, having a larger effect on the recommendations. As with the random attack, the target item is rated with the maximum rating value.
%
%\textbf{Bandwagon Attack:} This advanced attack model leverages Zipf's law distribution of popularity and then generates the biased profiles that contain frequently rated items~\cite{mobasher2007toward}. Here, filler items is a set of most frequently rated items. The rating value for each filler item is drawn from a normal distribution around the mean rating value across the whole dataset. Similar to random and average attack, the maximum rating value is assigned to the target item.
%
%\textbf{Co-visitation Attack:} This is the state-of-the-art attack against co-visitation based recommender systems. This attack is performed by injecting fake co-visitations between a target item and carefully selected filler items. The attack goal can be prompting or demoting a selected item. We allow each fake user to inject $n$ fake co-visitations in this attack.

%\subsection{Experimental Design}
%
%In this section, we evaluate the performance of our proposed data poisoning attacks model. Our goal is to answer the following research questions:
%
%%\comment{TODO: Some of the questions no longer make sense now. Come up with a new set of %questions based on our experiment results.}
%
%\begin{enumerate}
%\item Is manipulating the recommendation list of top-$k$ most positive users indeed sufficient to affect the recommendation lists of a large number of users?
%
%\item How does the proposed attack algorithm perform on different types of recommender systems?
%
%\item How does the density of the user preference graphs affect performance of the proposed attack algorithm?
%
%\item How does the popularity of the target item affect performance of the proposed attack algorithm?
%
%\item How robust is the proposed attack algorithm against fake account detection?
%\end{enumerate}
%
%
%Our experiments are conducted on two real word datasets (Table~\ref{datasets}), which are commonly used for evaluation of recommender systems. We define the \textit{sparsity} of a dataset as follows:
%\begin{align}
%Sparsity = 1 - \frac{N_r}{|U| * |I|},
%\end{align}
%where $N_r$ is the total number of user ratings included in the dataset. The first dataset we used is \textbf{MovieLens 100K (Movie)}. This dataset consists of 943 users, 1,682 movies and 100,000 ratings. The sparsity of Movie is 93.67\%. The second dataset we use is \textbf{Amazon Instant Video (Video)}. The original dataset contains 400k users, 20k instant videos and 500k ratings. For our experiments, we discard the users who have rated less than 6 instant videos. This resulted in 5,073 users, 10,843 items and 48,843 ratings. The sparsity of this dataset is 99.91\%.
%

%For all the attacks, we generate a number of attack profiles and insert them into the system and then generate predictions. Let $m/|U|$ be the \textit{attack size}, which is the ratio between the number of inserted attack profiles and the whole normal profiles in the rating database. If there are 1,000 users in the dataset, so an attack size of 1\% corresponds to 10 attack profiles added to the system.

%We use hit ratio $h(t)$ as our evaluation metric, and design four tasks to evaluate the performance of our proposed data poisoning attacks, which are described below.

%\textbf{Data Poisoning Attack:} We randomly select 10 items from the dataset as target items, and the goal of our attack is to maximize $h(t)$. Each of these items is attacked individually, and the average $h(t)$ is reported in the experiment.
%
%\textbf{Cold-Start Item Problem:} The goal of this attack is also to maximize target items' hit ratio. We also random select 10 items as our target items, but each item is a ``cold" item that has been rated by no more than 5 users. Attack is also performed on each item individually. Through this task, we want to show that our attack can effectively handle the cold-start problem in launching attacks to recommender systems.

%\textbf{Evolving Attack:} In this section, we consider an evolving attack scenario, which existing normal users could add authentic data into the dataset while attacker is attacking the system. This is closer to real-word situation because the real-word data is changing all the time. We select the same targets as data poisoning attacks and show that our attack model still achieve a good performance under evolving dataset.







%\begin{table*}[ht]
%	\centering
%	\caption{HR@10 Comparisons of Different Models for Cold-Start Item Problem.}\label{coldStartResults}
%	\begin{tabular}{cc|cccc}
%		\hline
%		Datasets & Attack Size & 0.5\% & 1\%   & 3\%   & 5\% \bigstrut\\
%		\hline
%		\hline
%		\multirow{6}[2]{*}{Movie} & None  & 0     & 0     & 0     & 0 \bigstrut[t]\\
%		& Our method & \textbf{0.0005} & \textbf{0.0042} & \textbf{0.0104} & \textbf{0.0131} \\
%		& Average & 0     & 0     & 0     & 0 \\
%		& Bandwagon & 0     & 0     & 0     & 0 \\
%		& Random & 0     & 0     & 0     & 0 \\
%		& Co-visitation &   0    &   0    &    0.0005   &  0.0027 \bigstrut[b]\\
%		\hline
%		\multirow{6}[2]{*}{Video} & None  & 0.0001 & 0.0001 & 0.0001 & 0.0001 \bigstrut[t]\\
%		& Our method & \textbf{0.0285} & \textbf{0.0576} & \textbf{0.1727} & \textbf{0.2845} \\
%		& Average & 0.0148 & 0.0323 & 0.1358 & 0.2554 \\
%		& Bandwagon & 0.0130 & 0.0314 & 0.1305 & 0.2481 \\
%		& Random & 0.0137 & 0.0317 & 0.1323 & 0.2500 \\
%		& Co-visitation &   0.0135    &   0.0313    &   0.1333    & 0.2539 \bigstrut[b]\\
%		\hline
%		\hline
%	\end{tabular}%
%\end{table*}%


%\begin{table*}[ht]
%	\centering
%	\caption{HR@10 for different atta.}\label{Evolving_attack}
%	\begin{tabular}{cc|cccc}
%		\hline
%		Datasets & Attack Size & 0.5\% & 1\%   & 3\%   & 5\% \bigstrut\\
%		\hline
%		\hline
%		\multirow{6}[2]{*}{Movie} & None  & 0.0022 & 0.0022 & 0.0022 & 0.0022 \bigstrut[t]\\
%		& Our method & \textbf{0.0055} & \textbf{0.0067} & \textbf{0.0138} & \textbf{0.0200} \\
%		& Average & 0.0018 & 0.0020 & 0.0030 & 0.0043 \\
%		& Bandwagon & 0.0018 & 0.0021 & 0.0030 & 0.0042 \\
%		& Random & 0.0018 & 0.0020 & 0.0027 & 0.0044 \\
%		& Co-visitation &  0.0020     &    0.0021    &    0.0030    &  0.0044 \bigstrut[b]\\
%		\hline
%		\multirow{6}[2]{*}{Video} & None  & 0.0019 & 0.0019 & 0.0019 & 0.0019 \bigstrut[t]\\
%		& Our method & \textbf{0.0325} & \textbf{0.0633} & \textbf{0.1859} & \textbf{0.3204} \\
%		& Average & 0.0152 & 0.0321 & 0.1317 & 0.2661 \\
%		& Bandwagon & 0.0133 & 0.0301 & 0.1272 & 0.2536 \\
%		& Random & 0.0138 & 0.0298 & 0.1273 & 0.2606 \\
%		& Co-visitation &   0.0140     &   0.0309    &  0.1288     & 0.2622 \bigstrut[b]\\
%		\hline
%		\hline
%	\end{tabular}%
%\end{table*}%




\begin{table*}[ht]
	\centering
	\caption{HR@10 for different  attacks with different attack sizes. }\label{Data_poisoning_attacks_Results}
	\begin{tabular}{c|c|cccc|cccc}
		\hline
		\multirow{3}[6]{*}{Dataset} & \multirow{3}[6]{*}{Attack } & \multicolumn{8}{c}{Attack size} \bigstrut\\
		\cline{3-10}          &       & \multicolumn{4}{c|}{Random target items} & \multicolumn{4}{c}{Unpopular target items  } \bigstrut\\
		\cline{3-10}          &       & 0.5\% & 1\%   & 3\%   & 5\%   & 0.5\% & 1\%   & 3\%   & 5\% \bigstrut\\
		\hline
		\hline
		\multirow{6}[2]{*}{Movie} & None  & 0.0022 & 0.0022 & 0.0022 & 0.0022 & 0     & 0     & 0     & 0 \bigstrut[t]\\
		& Random & 0.0028 & 0.0030 & 0.0038 & 0.0052 & 0     & 0     & 0     & 0 \\
		& Average & 0.0027 & 0.0030 & 0.0038 & 0.0049 & 0     & 0     & 0     & 0 \\
		& Bandwagon & 0.0027 & 0.0030 & 0.0037 & 0.0048 & 0     & 0     & 0     & 0 \\
		& Co-visitation & 0.0030 & 0.0030 & 0.0037 & 0.0050 & 0     & 0     & 0.0005 & 0.0027 \\
		& Our attack & \textbf{0.0040} & \textbf{0.0069} & \textbf{0.0134} & \textbf{0.0168} & \textbf{0.0005} & \textbf{0.0042} & \textbf{0.0104} & \textbf{0.0131} \bigstrut[b]\\
		\hline
		\multirow{6}[2]{*}{Video} & None  & 0.0019 & 0.0019 & 0.0019 & 0.0019 & 0.0001 & 0.0001 & 0.0001 & 0.0001 \bigstrut[t]\\
		& Random & 0.0181 & 0.0377 & 0.1456 & 0.2692 & 0.0137 & 0.0317 & 0.1323 & 0.2500 \\
		& Average & 0.0185 & 0.0397 & 0.1472 & 0.2775 & 0.0148 & 0.0323 & 0.1358 & 0.2554 \\
		& Bandwagon & 0.0171 & 0.0372 & 0.1443 & 0.2660 & 0.0130 & 0.0314 & 0.1305 & 0.2481 \\
		& Co-visitation & 0.0180 & 0.0378 & 0.1460 & 0.2688 & 0.0135 & 0.0313 & 0.1333 & 0.2579 \\
		& Our attack & \textbf{0.0323} & \textbf{0.0625} & \textbf{0.1828} & \textbf{0.2966} & \textbf{0.0285} & \textbf{0.0576} & \textbf{0.1727} & \textbf{0.2845} \bigstrut[b]\\
		\hline
		\hline
	\end{tabular}%
\end{table*}%


\begin{table}[ht]
	\centering
	\caption{HR@$N$ for different $N$.}\label{TOPN}
	\addtolength{\tabcolsep}{-2pt}

	\begin{tabular}{c|c|ccccc}
		\hline
		\multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{Attack} & \multicolumn{5}{c}{$N$} \bigstrut\\
		\cline{3-7}          &       & 1     & 5     & 10    & 15    & 20 \bigstrut\\
		\hline
		\hline
		\multirow{6}[2]{*}{Movie} & None  & 0     & 0.0001 & 0.0022 &  0.0060 & 0.0085 \bigstrut[t]\\
		& Random & 0     & 0.0004 & 0.0038 & 0.0076 & 0.0109 \\
		& Average & 0     & 0.0005 & 0.0038 & 0.0077 & 0.0112 \\
		& Bandwagon & 0     & 0.0004 & 0.0037 & 0.0076 & 0.0109 \\
		& Co-visitation & 0     & 0.0007 & 0.0040 & 0.0074 & 0.0108 \\
		& Our attack & \textbf{0.0024} & \textbf{0.0066} & \textbf{0.0134} & \textbf{0.0193} & \textbf{0.0243} \bigstrut[b]\\
		\hline
		\multirow{6}[2]{*}{Video} & None  & 0.0001 & 0.0008 & 0.0019 & 0.0036 & 0.0047 \bigstrut[t]\\
		& Random & 0.0461 & 0.0989 & 0.1456 & 0.1820 & 0.2130 \\
		& Average & 0.0476 & 0.1019 & 0.1472 & 0.1840 & 0.2144 \\
		& Bandwagon & 0.0454 & 0.0975 & 0.1443 & 0.1783 & 0.2090 \\
		& Co-visitation & 0.0479 & 0.1018 & 0.1463 & 0.1835 & 0.2131 \\
		& Our attack & \textbf{0.0665} & \textbf{0.1359} & \textbf{0.1828} & \textbf{0.2116} & \textbf{0.2314} \bigstrut[b]\\
		\hline
		\hline
	\end{tabular}%
\end{table}%


\subsection{Attacking Graph-based Systems}
We first consider the white-box setting, i.e., the graph-based recommender system and its restart probability are known to the attacker. 

\myparatight{Impact of attack size} Table~\ref{Data_poisoning_attacks_Results} shows the results for the compared poisoning attacks with different attack sizes. The attack size means that the number of fake users is a certain fraction of the normal users, e.g., 1\% attack size means that the number of fake users is 1\% of the number of normal users. The row in ``None'' means the hit ratios without any attacks. First, our attack can effectively promote target items. For instance, in the Video dataset, when injecting 1\% fake users, the hit ratio of a random target item increases by around 33 times, while the hit ratio of an unpopular target item increases by around 580 times. Second, our attack is significantly more effective than existing attacks. For instance, in the Movie dataset, when injecting 1\% fake users, our attack improves the hit ratio upon the best compared attack by 2.3 times for a random target item, while our attack improves the hit ratio from 0 to 0.0042 for an unpopular target item. The reason is that random attack, average attack, and bandwagon attack are agnostic to recommender systems, while the co-visitation attack was specifically designed for association-rule-based recommender systems. 

Third, the hit ratio gain is more significant for unpopular target items than random target items. For instance, our attack improves the hit ratio by 96 times and 1700 times for a random target item and an unpopular target item respectively, when injecting 3\% fake users into the Video dataset. Fourth, all attacks are more effective on the Video dataset than the Movie dataset. We speculate the reason is that Video is more sparse, and thus is easier to attack. More specifically, when the dataset is more sparse, it is easier to inject fake users that are similar to a large number of normal users. 



%\noindent Table~\ref{Data_poisoning_attacks_Results} shows the results of data poisoning attacks. "None" means the $h(t)$ before attack, the same below. It can be seen that the proposed method significantly outperform all baselines at most of test points. Specifically, using the same attack size, our method can achieve a hit ratio that is much higher than the baselines on average. At certain test point, this difference is up to one to two orders of magnitude. This result demonstrates the effectiveness of our attacking strategy, i.e., attacking only the most influential users to maximize the impact on the other users' recommendation list. It can be seen that our method shows particularly good performance when the attack size is below 5\%. We argue that the advantage at smaller attack size is more preferable. This is due to the fact that real world recommender systems usually involves millions of users and items and hence using large attack size can be extremely expensive. For example, Amazon is reported to have more than 300 million users and YouTube has more than 1 billion. Launching an attack even of size 5\% means injecting 15 million fake accounts to Amazon or 50 million to YouTube, which is impractical.
%
%Our method is also the best performer on both two datasets. Recall that these two datasets have very different sparsity. In general, all the compared attacks achieved the best performance on the Video dataset. However, it is not clear that whether the relatively higher hit ratio of all attacks is a result of the higher sparsity or the larger user set. Regardless, the proposed method achieves the best average hit ratio. 



\myparatight{Impact of the number of recommended items} Table~\ref{TOPN} shows the hit ratios for different attacks when the recommender system recommends different numbers (i.e., $N$) of items to users, where random target items are used and the attack size is fixed to be 3\%. First, we observe that our attack is effective and is more effective than the existing attacks for different values of $N$. Second, when $N$ is smaller, the hit ratio gains of our attack over existing attacks are more significant. For instance, when $N=20$ and $N=5$, our attack's hit ratios improve upon the best existing attacks by twice and by 9.5 times in the Movie dataset, respectively. This indicates that our attack ranks the target item higher in the recommendation lists than existing attacks. The reason is that the Wilcoxon-Mann-Whitney loss function~\cite{backstrom2011supervised} adopted by our attacks aims to optimize the ranking performance of the target item.  



%\noindent Table~\ref{TOPN} is the result of different attack models with attack size 3\%. From Table~\ref{TOPN}, we know that our attack model can make precise recommendations with small attack size (3\%) and even when $N$ is small, e.g., $N=1$, which means we can successful market our target items to a large group of users accurately with little effort.


\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Result-filler-Movielens.pdf}
		\caption{Movie}
	\end{subfigure}
	%\hskip1em
	\begin{subfigure}[b]{0.23\textwidth}
		\includegraphics[width=\textwidth]{Result-filler-Amazon.pdf}
		\caption{Video}
	\end{subfigure}
	\caption{Impact of the number of filler items.} \label{filler_para}
\end{figure}


\myparatight{Impact of the number of filler items} Figure~\ref{filler_para} shows the impact of the number of filler items on our attacks for random target items. On the Movie dataset, the hit ratio decreases as the attacker uses more filler items. However, on the Video dataset, the hit ratio increases and fluctuates as more filler items are used. Therefore, the relationship between the hit ratio and the number of filler items heavily depends on datasets. We note that Mobasher et al.~\cite{mobasher2007toward} had similar observations for the average and bandwagon attacks. Intuitively, an attacker should be more powerful and achieve better hit ratios when using more filler items. Our results and previous study~\cite{mobasher2007toward} show that this intuition does not hold. Understanding such phenomena theoretically is an interesting future work. 

%We believe that it is an interesting future work to study 

%\noindent We also investigate the impact of the number of filler items on our proposed model. From Fig.~\ref{filler_para}, we see that increasing the number of filler items does not necessarily results in a better attack impact, since most normal users will only rate a small number of items. An attacker, therefore, only needs to rate a small part of the items to make the attack effective.




%\subsubsection{Cold-Start Item Problem}

%\comment{Need complete revision}

%\noindent Our proposed attack model has an interesting application for the cold-start item problem~\cite{lika2014facing} associated with newly released or less popular items, which is pervasive in real-world recommendation applications. It is well-known that MF-based method, or other collaborative filtering-based methods in general, perform poorly on cold-start items due to the lack of enough reviews and ratings for these items. Many efforts~\cite{menon2011response,zheng2017joint,lin2013addressing} have been made to mitigate the cold-start item problem, where a common theme among them is to exploit \textit{side information} such as user reviews~\cite{zheng2017joint} and social network~\cite{lin2013addressing}. However, these methods become infeasible when such side information is not available and it is hard to choose the best auxiliary information in reality. To the best of our knowledge, few work have tackled the cold-start item problem fully within the scope of data poisoning attacks which relies exclusively on the available rating information. Using our proposed data poisoning attacks model, when a ``new'' item is introduced, the company/vendor has the opportunity to market it to the positive users and have the system recommend it to other users. In this experiment, we randomly select 10 ``new'' target items with the intent of addressing the cold-start item problem. In our experiment, each target item has been rated by no more than 5 users, and attack is performed on each item individually. Table~\ref{coldStartResults} shows the evaluation results of different attack models for cold-start item problem. From Table~\ref{coldStartResults}, we know that our proposed data poisoning attacks model significantly outperforms all baselines for the cold-start item problem. Besides the observations we made in the data poisoning attacks problem, we have some other interesting findings.
%
%From Table~\ref{Data_poisoning_attacks_Results} and Table~\ref{coldStartResults}, we know that the ratings distribution of the target item influences attack performance. A low popularity item is easier to attack compared to a popular item. Because an item has few ratings is more ``volatile'', it is easier to manipulate the recommendations for that item. Table~\ref{Data_poisoning_attacks_Results} and Table~\ref{coldStartResults} also show that the sparser the dataset, the easier to mount cold-start items in that dataset. This is because sparser dataset has more unpopular items compared to denser dataset in general, thus is easier to promote a cold target item. 
%
%\subsubsection{Evolving Attack} 
%
%\noindent In this section, we consider a evolving attack scenario, which existing normal users could add authentic data into the dataset in the window between two consecutive fake user injections. This is closer to real-world situation, because the real-world data is dynamic and changing all the time. While the attacker is learning and inserting fake data into the dataset, existing normal users may also buy/rate some items. Attackers do not know the normal users' behavior and normal users do not know the attackers'. In this section, we assume the number of added authentic ratings is the same as the number of added fake ratings. Because each fake user will rate the target item as well as $n$ filler items, then in the window between two consecutive fake user injections, we also add $n + 1$ authentic ratings into the dataset. Since a existing normal user does not rate many items at one time under normal circumstances, thus we random select $n + 1$ normal users and each normal user randomly rate one item if this user has not rated the item before. The rating each normal user give to its select item is drawn from a normal distribution around the mean rating for this item. From Table~\ref{Evolving_attack}, we know that, our proposed attack model achieves a better attack performance under evolving attack compared to original data poisoning attacks. This makes sense because if we add authentic data while attacking, attackers gain more information about the data, including original rating data, previous added authentic data and fake data, thus attackers could learn a more accurately attack model and easier attack the target items. From Table~\ref{Evolving_attack}, we also know that all baselines perform worse in evolving attack case, because all baselines random select the filler items, as the dataset increase, it is harder for them to attack the target item. In conclusion, we know that our attack model is more suitable to evolving attack.



\subsection{Transferring to Other Systems}

In the previous section, we assume that the attacker has a \emph{white-box} access to the target recommender system. In this section, we consider an attacker has a \emph{gray-box} and \emph{black-box} access to the recommender system. In particular, in the gray-box setting, the recommender system is still graph-based recommender system, but the key parameter \emph{restart probability $\alpha$} is unknown to the attacker. In the black-box setting, the attacker does not know the target recommender system algorithm. To simulate such black-box setting,  we assume the attacker generates fake users based on a graph-based recommender system, while the target recommender system uses matrix factorization. 

 \begin{figure}[!t]
	\centering
		\includegraphics[width=0.45\textwidth]{Result-restart-Movielens.pdf}
%		\caption{Movie}
%	\end{subfigure}
%	%\hskip1em
%	\begin{subfigure}[b]{0.23\textwidth}
%		\includegraphics[width=\textwidth]{Result-restart-Amazon.pdf}
%		\caption{Video}
%	\end{subfigure}
	\caption{Hit ratio of our attack as a function of the restart probability of the target graph-based recommender system under the gray-box setting.} 
	\label{restart_para}
\end{figure}



\myparatight{Gray-box setting} The attacker uses a restart probability $\alpha=0.3$ in graph-based recommender system to generate fake users. Figure~\ref{restart_para} shows the hit ratios for random target items of our attacks when the target graph-based recommender system uses different restart probabilities.  We observe that the hit ratio reaches the maximum when the restart probability is 0.3. The reason is that the attacker also sets the restart probability to be 0.3, which essentially reduces to a white-box attack. When the target recommender system uses a 
restart probability other than 0.3, our attack is less effective. However, our attack is still much more effective than existing attacks (please refer to Table~\ref{Data_poisoning_attacks_Results}). 

%\textbf{Restart Probability $\alpha$:} In this scenario, the attackers know the recommender algorithm, but does not know certain parameters of the algorithm, e.g., restart probability $\alpha$ of RWR. In this experiment, we fix the restart probability of our attack model as $\alpha = 0.3$, and vary the $\alpha$ of recommender algorithm (RWR). From Fig.~\ref{restart_para}, we know that our attack model is not sensitive to the parameter of restart probability $\alpha$. In Movie dataset, $\alpha = 0.3$ achieves the best attack performance, and $\alpha = 0.1$ performs worst, but it still outperforms all baselines. In Video dataset, out attack model also achieves a good attack impact in different settings of $\alpha$. So even though we do not know the exact restart probability $\alpha$ of given recommender system, we could still achieve a good attack performance by guessing the $\alpha$ randomly.


\myparatight{Black-box setting} We assume the attacker generates fake users using a graph-based recommender system, while the target recommender system uses matrix factorization.  In particular, we use the popular matrix factorization technique proposed in~\cite{MFRec09} to implement the target recommender system. Table~\ref{MF_attack} shows the hit ratios of our attacks and existing attacks for random target items. First, all compared attacks can transfer to matrix factorization based recommender systems, especially on the Video dataset. Specifically, all attacks significantly improve the hit ratios of target items upon no attacks on the Video dataset. However, the hit ratio gains on the Movie dataset is less significant. We suspect the reason is that the Movie dataset is denser and is harder to attack. 

Second, the differences between our attack and the existing attacks are small, which means that different attacks have similar \emph{transferability} to matrix factorization based recommender systems.   
Third, the hit ratio gains of all attacks are less (or more) significant in the black-box setting than in the white-box setting on the Movie (or Video) dataset (comparing Table~\ref{Data_poisoning_attacks_Results} and Table~\ref{MF_attack}). For instance, on the Movie dataset, our attack improves the hit ratio over no attacks by 3 times and by 20\%  in the white-box setting and black-box setting, respectively, when the attack size is 1\%. However, on the Video dataset, our attack improves the hit ratio over no attacks by 33 times and 4000 times  in the white-box setting and black-box setting, respectively, when the attack size is 1\%. This is because matrix factorization is known to achieve better hit ratios when the dataset is denser~\cite{MFRec09}. For instance, matrix factorization achieves lower hit ratios than the graph-based recommender system on the Video dataset when there are no attacks. After the attacker adds fake users, the target item has dense rating scores and thus it is recommended to many users by matrix factorization. As a result, the poisoning attacks have even more significant hit ratio gains over no attacks in the black-box setting than in the white-box setting. 




\begin{table}[!t]
	\centering
	\caption{HR@10 under the black-box setting, where the attacker generates fake users using a graph-based recommender system while the target recommender system uses matrix factorization.}\label{MF_attack}
	\begin{tabular}{c|c|cccc}
		\hline
		\multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{Attack } & \multicolumn{4}{c}{Attack size} \bigstrut\\
		\cline{3-6}          &       & 0.5\% & 1\%   & 3\%   & 5\% \bigstrut\\
		\hline
		\hline
		\multirow{6}[1]{*}{Movie} & None  & 0.0104 & 0.0104 & 0.0104 & 0.0104 \bigstrut[t]\\
		& Random & \textbf{0.0116} & \textbf{0.0125} & 0.0144 & 0.0198 \\
		& Average & \textbf{0.0116} & \textbf{0.0125} & 0.0144 & 0.0196 \\
		& Bandwagon & \textbf{0.0116} & \textbf{0.0125} & 0.0144 & 0.0198 \\
		& Co-visitation & 0.0015 & \textbf{0.0125} & 0.0144 & 0.0196 \\
		& Our attack & \textbf{0.0116} & 0.0124 & \textbf{0.0169} & \textbf{0.0226} \\
		\hline
		\multirow{6}[1]{*}{Video} & None  & 0.0001 & 0.0001 & 0.0001 & 0.0001 \\
		& Random & 0.0336 & 0.4142 & 0.5771 & 0.5884 \\
		& Average & 0.0317 & 0.4149 & \textbf{0.5776} & \textbf{0.5895} \\
		& Bandwagon & 0.0329 & 0.4142 & 0.5773 & 0.5883 \\
		& Co-visitation & 0.0325 & 0.4145 & 0.5775 & 0.5886 \\
		& Our attack & \textbf{0.0340} & \textbf{0.4158} & 0.5767 & 0.5852 \bigstrut[b]\\
		\hline
		\hline
	\end{tabular}%
\end{table}%


%In this situation, the attackers do not know the exact algorithm of recommender system. Because our default recommender algorithm is RWR, so in order to attack other recommender algorithms, we first generate fake users on RWR algorithm, we then run other recommender algorithm (e.g., matrix factorization) on the rating data after injecting fake users. In this paper, we use the popular MF technique presented in ~\cite{MFRec09}. Here, the number of latent factors is 5, and the regularization coefficient is set to 0.007. From Table~\ref{MF_attack}, we know that the clear advantage of our method is observed not only on the random walk based recommender system, but also the matrix factorization based system, despite the fact that our method is not specifically tailor for the latter. When applied on MF-based system, the advantage of our method is not as drastic as on RWR based system, but is still obvious. Besides, all of the attack models perform poorly for cold-start item problem when the recommender system is MF, this is mainly because MF algorithm suffers from cold-start item problem~\cite{MFRec09}. In particular, a MF based collaborative recommender finds it difficult to make good predictions for new items, which have few ratings.


\begin{table*}[ht]
	\centering
	\caption{Detection results for different attacks.}\label{Detection_resultsl}
	\begin{tabular}{c|c|cccc|cccc}
		\hline
		\multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{Attack} & \multicolumn{4}{c|}{FPR}       & \multicolumn{4}{c}{FNR} \bigstrut\\
		\cline{3-10}          &       & 0.5\% & 1\%   & 3\%   & 5\%   & 0.5\% & 1\%   & 3\%   & 5\% \bigstrut\\
		\hline
		\hline
		\multirow{5}[2]{*}{Movie} & Random & 0.0458 & \textbf{0.0477} & 0.0463 & 0.0483 & 0     & 0.2400 & 0.4367 & 0.4060 \bigstrut[t]\\
		& Average & 0.0468 & 0.0463 & 0.0478 & 0.0475 & 0     & 0.2300 & \textbf{0.4567} & 0.4140 \\
		& Bandwagon & {0.0414} & {0.0417} & {0.0415} & {0.0445} & 0     & 0.1900 & 0.4100 & 0.3400 \\
		& Co-visitation & 0.0437 & 0.0460 & 0.0454 & 0.0461 & 0     & 0.2400 & 0.4200 & 0.3950 \\
		& Our attack & \textbf{0.0479} & 0.0474 & \textbf{0.0483} & \textbf{0.0493} & \textbf{0.1600} & \textbf{0.3900} & \textbf{0.4567} & \textbf{0.4220} \bigstrut[b]\\
		\hline
		\multirow{5}[2]{*}{Video} & Random & {0.0719} & 0.0717 & 0.0706 & 0.0719 & \textbf{0.2520} & 0.2820 & 0.3773 & 0.5116 \bigstrut[t]\\
		& Average & 0.0721 & 0.0700 & {0.0698} & {0.0693} & 0.2120 & \textbf{0.2860} & \textbf{0.3820} & \textbf{0.5452} \\
		& Bandwagon & 0.0721 & {0.0699} & 0.0701 & 0.0702 & 0.2040 & 0.2740 & 0.3467 & 0.5404 \\
		& Co-visitation & {0.0719} & 0.0705 & 0.0705 & 0.0702 & 0.2105 & 0.2850 & 0.3747 & 0.5369 \\
		& Our attack & \textbf{0.0730} & \textbf{0.0729} & \textbf{0.0725} & \textbf{0.0725} & 0.1880 & 0.2220 & 0.3353 & 0.5000 \bigstrut[b]\\
		\hline
		\hline
	\end{tabular}%
\end{table*}%


\begin{table}[ht]
	\centering
	\caption{HR@10 for different attacks when the service provider deploys a classifier to predict fake users and excludes the predicted fake users from the  system.}\label{attackUnderDetection}
	\begin{tabular}{c|c|cccc}
		\hline
		\multirow{2}[4]{*}{Dataset} & \multirow{2}[4]{*}{Attack } & \multicolumn{4}{c}{Attack size} \bigstrut\\
		\cline{3-6}          &       & 0.5\% & 1\%   & 3\%   & 5\% \bigstrut\\
		\hline
		\hline
		\multirow{6}[1]{*}{Movie} & None  & 0     & 0     & 0     & 0 \bigstrut[t]\\
		& Random & 0     & 0     & 0.0011 & 0.0031 \\
		& Average & 0     & 0     & 0.0014 & 0.0032 \\
		& Bandwagon & 0     & 0     & 0     & 0.0016 \\
		& Co-visitation & 0     & 0     & 0.0009 & 0.0027 \\
		& Our attack & 0     & \textbf{0.0024} & \textbf{0.0066} & \textbf{0.0109} \\
		\hline
		\multirow{6}[1]{*}{Video} & None  & 0.0008 & 0.0008 & 0.0008 & 0.0008 \\
		& Random & 0.0046 & 0.0087 & 0.0713 & 0.1530 \\
		& Average & 0.0058 & 0.0098 & 0.0891 & 0.1509 \\
		& Bandwagon & 0.0032 & 0.0071 & 0.0772 & 0.1459 \\
		& Co-visitation & 0.0025 & 0.0077 & 0.0739 & 0.1515 \\
		& Our attack & \textbf{0.0064} & \textbf{0.0197} & \textbf{0.1028} & \textbf{0.1788} \bigstrut[b]\\
		\hline
		\hline
	\end{tabular}%
\end{table}%


\section{Detecting Fake Users}
Detecting fake users is closely related to \emph{Sybil detection} in social networks. Many methods have been developed for Sybil detection. 
These methods leverage IP addresses (e.g.,~\cite{EVILCOHORTSecurity15}), user behavior (e.g.,~\cite{Wang13Clickstream}), or social relationships between users (e.g.,~\cite{sybilbelief,wang2017gang,wang2018structure}). Since we do not have access to IP addresses nor social relationships of users, we explore a behavior based method. 
In particular, we extract a set of features from a user's rating scores and train a binary classifier to classify users to be normal or fake. We will also study the effectiveness of the poisoning attacks when the recommender system has deployed such a detector to predict fake users and has excluded the predicted fake users from the recommender system. 

\myparatight{Rating scores based detection} Intuitively, the fake users' rating scores are generated in specific ways, and thus it may be possible to distinguish between normal users and fake users using their rating scores. Indeed, previous studies~\cite{chirita2005preventing,mobasher2007toward} extracted several features from rating scores to train a binary classifier to distinguish between normal users and fake users. We adopt these features in our work. Specifically, the features are as follows. 



%\textbf{Detection and Attack after Detection:} Real world recommender system usually employs certain countermeasures against shilling attacks. Attempting to detect fake user ratings is one of the most common countermeasure. As attackers gain limited knowledge about the recommender systems, attack profiles differ from that of normal profiles in a statistical way. The difference is mainly because of two reasons: the rating given to the target item, and the rating distribution among the filler items. There are several detection attributes that have been proposed~\cite{chirita2005preventing,mobasher2007toward} to measure these differences. In this section, we will use the following five attributes to detect the attack profiles, namely, RDMA~\cite{chirita2005preventing}, WDA~\cite{mobasher2007toward}, WDMA~\cite{mobasher2007toward}, MeanVar~\cite{mobasher2007toward} and FMTD~\cite{mobasher2007toward}. We then use KNN classification algorithm to detect attack profiles based on the above five attributes and delete the suspicious attack profiles. After that, we run the recommender algorithm on the remaining rating data and show the performance of different attack models under detection.

\begin{itemize}
	\item \textit{Rating Deviation from Mean Agreement} (RDMA)~\cite{chirita2005preventing}: This feature measures the average deviation of a user's rating scores to the mean rating scores of the corresponding items. Formally, for a user $u$, RDMA is computed as follows:
	\begin{align}
	RDM{A_u} = \frac{{\sum\limits_{i \in {I_u}} {\frac{{|{r_{ui}} - \overline {r_i}|}}{{{o_i}}}}}}{{|{I_u}|}},
	\end{align}
	where ${{I_u}}$ is the set of items that user $u$ has rated, ${\left| {{I_u}} \right|}$ is the number of items in ${{I_u}}$, $r_{ui}$ is the rating score that $u$ gave to item $i$, $\overline {r_i}$ is the average rating score for item $i$, and $o_i$ is the total number of ratings  for item $i$.
	
	\item \textit{Weighted Degree of Agreement} (WDA)~\cite{mobasher2007toward}: This feature is simply the numerator of the RDMA feature, i.e., this feature is computed as follows:
	\begin{align}
	WD{A_u} = \sum\limits_{i \in {I_u}} {\frac{{|{r_{ui}} - \overline {r_i}|}}{{{o_i}}}}.
	\end{align}
	\item \textit{Weighted Deviation from Mean Agreement} (WDMA)~\cite{mobasher2007toward}: This feature is also based on RDMA, but it puts higher weights on rating deviations for items that have less ratings. The WDMA feature for a user $u$ is calculated as follows:
	\begin{align}
	 WDM{A_u} = \frac{{\sum\limits_{i \in {I_u}} {\frac{{|{r_{ui}} - \overline {r_i}|}}{{o_i^2}}} }}{{|{I_u}|}}.
	\end{align}
	
	\item \textit{Mean Variance} (MeanVar)~\cite{mobasher2007toward}: This feature measures the average variance of a user's rating scores to the mean rating scores of the corresponding items. Specifically,  the MeanVar feature for a user $u$ is given by:
	\begin{align}
	MeanVa{r_u} = \frac{{\sum\limits_{i \in {I_{u}}} {{{({r_{ui}} - \overline {r_i})}^2}} }}{{|{I_u}|}}.
	\end{align}
%	where ${I_{uF}}$ is the set of items in $I_u$ that are not given the maximum rating $r_{max}$ by user $u$.
	
	\item \textit{Filler Mean Target Difference} (FMTD)~\cite{mobasher2007toward}: This feature measures the divergence between a user's rating scores, and it is computed as follows:
	\begin{align}
	FMT{D_u} = \left| {\frac{{\sum\limits_{i \in {I_{uT}}} {{r_{ui}}} }}{{|{I_{uT}}|}} - \frac{{\sum\limits_{j \in {I_{uF}}} {{r_{uj}}} }}{{|{I_{uF}}|}}} \right|,
	\end{align}
	where ${I_{uT}}$ is the set of items in $I_u$ that $u$ gave the maximum rating score and ${I_{uF}}$ includes all other items in $I_u$.
	
\end{itemize}




%We consider a strong recommender system that knows the poisoning attack. In practice, the recommender system may not know the poisoning attack because an attacker could design specialized attacks. Therefore, our detection results represent an attacker could use  
For each poisoning attack, the service provider generates some fake users using the attack and labels some normal users as a training dataset. In our experiments, we generate 150 fake users (these fake users could be different from the fake users an attacker synthesizes when performing attacks) and sample 150 normal users as the training dataset. Then, using the above features, the service provider learns a KNN classifier, where $K$ is determined via cross-validation in the training dataset. % Note that the classifier could be different for different poisoning attacks.  


%\subsubsection{Detection and Attack after Detection Results} \noindent This section mainly contains two phases. In the first phase, we want to show the robustness of different attack models, that is how well the classification algorithm detect attack. In the second phase, we delete all detected fake users, and run recommender algorithm on the remaining data, we want to show the attack performance after detection.

\myparatight{Results of detecting fake users} We apply the classifiers to detect fake users generated by different poisoning attacks. We use \emph{False Positive Rate (FPR)} and \emph{False Negative Rate (FNR)} to measure the detection performance. Specifically, FPR is the fraction of normal users that are predicted to be fake, while FNR is the fraction of fake users that are predicted to be normal.  


Table~\ref{Detection_resultsl} shows the FPR and FNR when detecting the fake users generated in our experiments in Section~\ref{sec:exp} under the default parameter setting. We observe that a small fraction of normal users are predicted to be fake. When the service provider excludes the predicted fake users from the recommender system, these normal users won't receive \emph{personalized} recommendations from the recommender system. The service provider could leverage other methods to recommend items for such users, e.g., the service provider always recommends popular items to them (such recommendation is not personalized). Moreover, the detector misses a large fraction of fake users, i.e., FNR is large. Moreover, the FNR tends to increase as the attacker injects more fake users. A possible reason is that more fake users have more diverse patterns, and thus it is harder to detect them. 




%In this section, we use a separate defender (KNN supervised classification algorithm) to detect attack profiles based on the above five attributes, namely, RDMA, WDA, WDMA, MeanVar and FMTD. We assume defenders have full knowledge of the attack algorithms, and we train a defender for every attack algorithm. More precisely, for every poisoning data attacks method, we first use this attack method to separately generate 150 fake users (about 3\% attack size of Video dataset), then we train a KNN classifier based on these 150 fake users and another 150 uniform selected normal users. Based on the training data, KNN with $K=9$ is used to make a binary classifier. We then use the trained KNN classifier to detect the attacked profiles generated by its corresponding attack method in the data poisoning attacks task. Specially, in the detection phase, the classifier may misclassify some normal users as fake users. In this section, we use False Positive Rate (FP) and False Negative Rate (FN) show how different attack models could against detection, where FP is the fraction of normal users that are predicted to be fake and FN is the fraction of fake users that are predicted to be normal. From Table~\ref{Detection_resultsl}, we know that our proposed data poisoning attacks model admits a lower FN value, this is because our model is a heuristic algorithm, so fake users may easier to be detected compared to baselines, which randomly choose the filler items.

\myparatight{Attack effectiveness when detector is deployed} Suppose the service provider deploys the classifier to detect fake users. In particular, the service provider excludes the predicted fake users from the recommender system. Note that a small fraction of normal users will be excluded from the recommender system, while a large fraction of fake users will still be included in the recommender system. We re-compute the recommended items for each remaining user after excluding the predicted fake users from the recommender system and re-compute the hit ratios of the target items. The hit ratio of a target item is the fraction of the remaining normal users whose recommended items include the target item. 

Table~\ref{attackUnderDetection} shows the hit ratios of random target items for the compared poisoning attacks under the white-box setting.  First, we observe that these attacks are still effective in many cases. This is because a large fraction of fake users are not detected. Second, compared to the case where the service provider does not detect fake users, the hit ratios  are smaller (comparing Table~\ref{attackUnderDetection} with Table~\ref{Data_poisoning_attacks_Results}). The reason is that a large fraction of fake users are detected and excluded from the recommender system.  Third, our attack still substantially outperforms existing attacks. 

%In this section, we delete all fake users (including misclassified normal users and true fake users) detected in the test data in the detection phase, then perform recommender algorithm on the remaining attacked data. We show from Table~\ref{attackUnderDetection} that our attack model still outperforms all baselines even after detection. From Table~\ref{attackUnderDetection}, we know that by maximizing each fake user's attack impact and mimic normal user behaviors to avoid potential detection, our proposed attack model still achieve a good attack performance after detection.

%\subsubsection{Detection and Attack after Detection} \noindent In this section, we first use KNN supervised classification algorithm to detect attack profiles based on the above five attributes, namely, RDMA, WDA, WDMA, MeanVar and FMTD. We then delete the suspicious attack profiles and run the recommender algorithm on the remaining rating data. In the detection phase, to minimize over fitting, we partition the rating data in half. The first half is used as the training set and the second partition was used for testing. The training data is created by injecting fake users with attack size between 0.5\% and 5\%, and generating the detection attributes for normal and fake profiles. Based on the training data, KNN with $K=9$ is used to make a binary classifier. For each test, the second half of the data is injected with the same amount of fake users as the training data and we then run KNN classifier to detect fake users on the test data. Specially, in the detection phase, the classifier may misclassify some normal users as fake users. After that, we delete all fake users (including misclassified normal users and true fake users) detected in the test data and perform recommender algorithm on the remaining data. We show from Table~\ref{attackUnderDetection} that our attack model still outperform all baselines even under detection. From Table~\ref{attackUnderDetection}, we know that by maximizing each fake user's attack impact and mimic normal user behaviors to avoid potential detection, our proposed attack model still achieve a good attack performance under detection.






%\begin{figure}[t]
%	\centering
%	\begin{subfigure}[b]{0.23\textwidth}
%		\includegraphics[width=\textwidth]{Result-restart-Movielens.pdf}
%		\caption{Movie}
%	\end{subfigure}
%	%\hskip1em
%	\begin{subfigure}[b]{0.23\textwidth}
%		\includegraphics[width=\textwidth]{Result-restart-Amazon.pdf}
%		\caption{Video}
%	\end{subfigure}
%	\caption{Restart probability.} \label{restart_para}
%\end{figure}






==> arXiv - Copy/introduction.tex <==
%auto-ignore
\section{Introduction} \label{sec:intro}
% recommender system is important
%From e-business perspective, that the most valuable resource on the Internet is users' limited attention~\cite{simon1971designing}. On the other hand, customers frequently find themselves lost in an overwhelming number of choices when looking for products and services of their interests. As such, more and more users rely on \textit{recommender systems} to find items that best match their preferences. On the other hand, numerous web services (e.g., Amazon, eBay, YouTube, Tripadvisor) also rely on recommender systems to attract users and increase profit. Consequently, making accurate recommendation becomes a crucial task in e-commercial.

In the era of big data, a fundamental challenge is to locate the data that are relevant to a particular user. Recommender systems aim to address this challenge: given a user's historical behavior and social data, a recommender system finds the data that match the user's preference. Indeed, recommender systems are widely deployed by web services (e.g., YouTube, Amazon, and Google News)  to recommend users relevant items such as products, videos, and news. 
In particular, \emph{collaborative filtering based recommender systems}, which analyze the correlations between users' historical behavior data for making recommendations, are widely deployed due to their effectiveness and generality. Depending on the techniques used to capture the correlations between users' behavior data, collaborative filtering based recommender systems can further include \emph{matrix-factorization-based}~\cite{MFRec09}, \emph{association-rule-based}~\cite{mobasher2000automatic,davidson2010youtube}, and \emph{graph-based}~\cite{fouss2007random} recommender systems. For instance, matrix-factorization-based recommender systems are deployed by Netflix to recommend movies, association-rule-based recommender systems are deployed by YouTube to recommend videos~\cite{davidson2010youtube}, and graph-based recommender systems are deployed by eBay~\cite{eBay2013a,eBay2013b} and Huawei App Store (a big app store in China)~\cite{He15,Guo17}. 

%poisoning attacks to recommender systems. 

It is commonly believed that recommender systems recommend users items that match their personal interests. However, several studies~\cite{profileinjectionattacksMahony04,lam2004shilling,mobasher2007toward,poisoningattackRecSys16,yang2017fake} have demonstrated that recommender systems are vulnerable to \emph{poisoning attacks}, which inject fake data to a recommender system such that the recommender system makes recommendations as an attacker desires. For instance, an attacker can inject fake users with carefully crafted fake rating scores to a recommender system such that a target item is recommended to as many users as possible. Conventional poisoning attacks~\cite{profileinjectionattacksMahony04,lam2004shilling,mobasher2007toward} (also known as \emph{shilling attacks}) are agnostic to recommendation algorithms, i.e., they are not optimized to a certain type of recommender systems. Therefore, such attacks often achieve suboptimal performance when the recommendation algorithm is known. To address this limitation, recent studies~\cite{poisoningattackRecSys16,yang2017fake} proposed poisoning attacks that were optimized for a particular type of recommender systems. For instance,
 Li et al.~\cite{poisoningattackRecSys16} proposed poisoning attacks optimized for matrix-factorization-based recommender systems, while 
 Yang et al.~\cite{yang2017fake} proposed poisoning attacks optimized for association-rule-based recommender systems. However,  how to design optimized poisoning attacks to graph-based recommender systems is still an open problem. 


%Despite the important role played by recommender systems on the Internet. It has been shown that existing recommender systems are vulnerable to security attacks. A resourceful attacker can spoof recommender systems to make recommendations as the attacker desires. Several attacks have been studied in the literature, including pollution attacks, data poisoning attacks, and fake co-visitation injection attacks. These attacks can fool a system into recommending a target item to some victim users or the general public, and/or removing a target item from the recommendation list shown to certain users. Nevertheless, performing such attacks in large scale at considered a challenging task due to several factors:
%
%\begin{enumerate}
%\item Pollution attacks~\cite{CSRF} rely on cross-site request forgery (CSRF), which targets a specific set of victim users. However, it is hard to perform CSRF attack to the general public.
%\item Exisiting data poisoning attacks require injecting fake accounts into the system. However, injecting a large number of fake accounts makes it much easier to detect the attackers~\cite{mehta2009unsupervised}.
%\item Some data poisoning attacks depend on the so called seed users (e.g, power users~\cite{wilson2013power,seminario2014attacking}, most central users~\cite{goyal2012recmax}) to provide biased ratings for a particular item, which may be infeasible in reality (e.g., need to bribe these seed users or hack their accounts).
%\item Fake co-visitation injection attacks~\cite{yang2017fake} require knowledge of the items' co-visitation information, which are usually not available to the public.
%\end{enumerate}

%\textbf{2)}  \textbf{3)}  \textbf{4)} 

%our work
In this work, we aim to design poisoning attacks for graph-based recommender systems~\cite{fouss2007random,eBay2013a,eBay2013b,He15,Guo17}. A graph-based recommender system uses a \emph{user preference graph} to represent users' rating scores to items. 
%Given a user-item rating score matrix, where the entry $(u,i)$ is the rating score that user $u$ gave to item $i$ or 0 if $u$ did not rate $i$, a graph-based recommender system first transforms the rating score matrix to a \emph{user preference graph}. 
In the graph, a node is a user or an item, an edge between a user and an item means that the user rated the item, and the edge weight is the corresponding rating score. To make recommendations to a user, the recommender system performs a \emph{random walk} in the user preference graph, where the random walk starts from the user and jumps back to the user with a certain probability (called \emph{restart probability}) in each step. After the random walk converges, each item has a stationary probability that essentially characterizes the closeness between the item and the user. Finally, the system recommends the items that have the largest stationary probabilities to the user. 

%problem formulation
In our poisoning attacks, an attacker's goal is to \emph{promote} a target item, i.e., making a graph-based recommender system  recommend the target item to as many users as possible.  
Like most existing poisoning attacks to recommender systems~\cite{profileinjectionattacksMahony04,lam2004shilling,mobasher2007toward,poisoningattackRecSys16}, our attacks inject fake users with carefully crafted rating scores to the target recommender system to achieve the attack goal. Due to limited resources and to avoid detection, we assume an attacker can inject $m$ fake users at most and each fake user rates $n$ items at most. For convenience, we call the items, which a fake user rates, the user's \emph{filler items}. The key challenge is to determine the filler items and their rating scores for each fake user. 
To address the challenge, we formulate poisoning attacks to graph-based recommender systems as an optimization problem,  whose {objective function} is the \emph{hit ratio} of the target item (i.e., the fraction of normal users whose recommended items include the target item) and whose {constraints} are that at most $m$ fake users with at most $n$ filler items can be injected. Solving this optimization problem produces $m$ fake users that maximize the hit ratio of the target item. 

%solution
However, this optimization problem is computationally intractable because  1) the hit ratio is related to the fake users' rating scores in a very complex way, and 2) the rating scores are integer variables. To address the computational challenge, we propose several techniques to solve the optimization problem approximately. Specifically, we approximate the hit ratio using the items' stationary probabilities, which are used to make recommendations in graph-based recommender systems. Moreover, 
we relax the fake users' rating scores as continuous variables, solve the optimization problem, and then generate filler items and their integer rating scores based on  the continuous variables. Finally, we propose a projected gradient descent based method to solve the optimization problem with an approximate hit ratio and relaxed continuous variables. 


%evaluation
We evaluate our poisoning attacks and compare them with several existing attacks using two real-world datasets. First, we evaluate the attacks under the \emph{white-box setting}, i.e., the graph-based recommendation algorithm and its parameter (i.e., restart probability) are known to the attacker. We find that our attack can effectively enhance the hit ratio of a target item. For instance, when the  system recommends 10 items to each user and the number of injected fake users is 1\% of the number of normal users, our attack  could improve  the hit ratio of an unpopular target item by around 580 times. Moreover, our attack is significantly more effective than existing attacks for graph-based recommender systems. For instance, compared to the poisoning attack proposed by Yang et al.~\cite{yang2017fake}, our attack can improve the hit ratio from 0.0\% to 0.4\% for an unpopular target item. The reason is that existing attacks are not optimized for graph-based recommender systems.  Second, we evaluate the attacks under \emph{gray-box setting} (the graph-based recommendation algorithm is known but its parameter is unknown) and \emph{black-box setting} (the recommendation algorithm is unknown). We find that, in the gray-box setting, even if the attacker does not know the restart probability, our attack can still substantially improve the hit ratios of target items. In the black-box setting, we assume an attacker generates fake users based on a graph-based recommender system, while the target recommender system is based on matrix factorization. Our results show that our attacks can also transfer to matrix factorization based recommender systems. 


We also study detecting fake users via supervised machine learning techniques and their impact on the effectiveness of poisoning attacks. Intuitively, the rating scores of fake users are generated in specific ways, and thus it could be possible to distinguish between normal users and fake users using their rating scores. Specifically, we extract features from a user's rating scores and learn a binary classifier using a training dataset that includes both normal users and fake users. The binary classifier is then used to predict a user to be normal or fake. We find that a small fraction of normal users are falsely predicted to be fake, while a large fraction (20\%$\sim$50\%) of fake users are falsely predicted to be normal. The service provider could deploy such a detector to predict fake users and exclude the predicted fake users from the recommender system. We evaluate our poisoning attacks and existing attacks under such scenario. We find that the poisoning attacks are still effective when such a detector is deployed, and our attack is still more effective than existing attacks. The reason is that a large fraction of fake users are not detected. 

%present the first systematic study of data poisoning attacks on graph-based recommender systems. Unlike existing attack models that target one type of recommender systems in general, we show that the threat of an attack can be maximized by targeting a specific recommender system. Our approach is to formulate data poisoning attacks to a recommender system as an integer programming optimization problem and solve an optimal attacking strategy. Compared to state-of-the-art attacks, our data poisoning attacks does not suffer from the aforementioned limitations and can be performed at large scale. Our study complements existing research on recommender systems security, and more importantly, it shows that existing recommender systems are more vulnerable than state-of-the-art attacks have revealed. If shilling attacks are not addressed carefully, the attackers can easily manipulate the system produce any recommendation behavior he or she desires.
%
%Our major technical contribution is a novel random walk based data poisoning attacks algorithm that yields significant impacts by injecting a small number of fake users. We discover that, instead of injecting all fake accounts at the same time as existing attacks do, injecting only one account at a time can achieve the best attack outcome. This is because our algorithm ensures that when a fake account is injected, it will take into consideration the impact of all previously injected accounts. As such, each injected fake account can achieve its optimal impact. Our attack does not rely on the cooperation of seed users, which is usually hard to acquire in reality. Instead, we attempt to attack the seed users' recommendation lists directly, which in return leads to the target item being recommended to a large number of other users. Moreover, when promoting a target item, our attack is able to alleviate the cold-start item problem of recommender systems and successfully recommend the target item to the desired users. Although the proposed attack in designed with a focus on graph-based recommender system, we show it is effective on various types of recommender systems, including matrix based, random walk based, and co-visitation based systems. We summarize our main contributions as follows:

In summary, our contributions are as follows:
\begin{packeditemize}
\vspace{2mm}
\item We provide the first systematic study on poisoning attacks to graph-based recommender systems. We formulate poisoning attacks as an optimization problem and propose techniques to solve the optimization problem approximately.  

\vspace{2mm}
\item We extensively evaluate our attacks and compare them with existing attacks using two real-world datasets.  

\vspace{2mm}
\item We study detecting fake users using their rating scores and evaluate the effectiveness of poisoning attacks when such a detector is deployed.

\end{packeditemize}





==> arXiv - Copy/macros.tex <==
%auto-ignore
% The name of this file is ``macros.tex''
%

%
% TEX defaults
%
%
% frame 6.5 * 9
\textwidth 6.5in
\textheight 9in

% left/right margins
\oddsidemargin 0pt
\evensidemargin 0pt
\marginparwidth 1in
\marginparsep 0pt

% top margin
\topmargin -25pt
\headheight 10pt
\headsep 30pt
% \topskip 0pt

% foot margin
%\footheight 0pt
\footskip 27pt


% macros for commonly used special fonts
\newcommand{\IE}{{\it i.e.,}\ }
\newcommand{\EG}{{\it e.g.,}\ }
% single/double spacing
%\newcommand{\SS}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\DS}{\renewcommand{\baselinestretch}{1.6}\large\normalsize}
% reduce the space between lines
\newcommand{\Tight}{\renewcommand{\baselinestretch}{0.9}\large\normalsize}
\newcommand{\HalfTight}{\renewcommand{\baselinestretch}{0.95}\large\normalsize}
\newcommand{\MinorTight}{\renewcommand{\baselinestretch}{0.975}\large\normalsize}
% Page title (primarily for foils)
% (this was called \HH}
\newcommand{\PageTitle}[1]{{\newpage \begin{center}{\LARGE {\bf {#1}} } \end{center} } }

% remove spaces around section headers
%\newcommand{\Section}[1]{\vspace{-3ex}\section{#1}\vspace{-2ex}}
\newcommand{\Subsection}[1]{\vspace{-2ex}\subsection{#1}\vspace{-1ex}}
\newcommand{\Subsubsection}[1]{\vspace{-2ex}\subsubsection{#1}\vspace{-1ex}}

% go forward n lines (negative for backward move)
\newcommand{\VLine}[1]{\vspace{#1ex}}
% itemize and enumerate without spaces around/between items
\newenvironment{TightItem}{\vspace{-2ex}\begin{itemize}
  \setlength{\itemsep}{-0ex}}{\end{itemize}\vspace{-1ex}}
\newenvironment{TightEnum}{\vspace{-2ex}\begin{enumerate}
  \setlength{\itemsep}{-0ex}}{\end{enumerate}\vspace{-1ex}}
\newenvironment{TightDesc}{\vspace{-1ex}\begin{description}
  \setlength{\itemsep}{-0ex}}{\end{description}\vspace{-1ex}}
% set the page number (to the first argument)
\newcommand{\SetPageNo}[1]{\countdef\pageno=0 \pageno=#1}
% things to do
\newenvironment{Todo}{\begin{large}\begin{bf}********** things to do
    ********** \\}{\\ **********\end{bf}\end{large}}
% for discussion
\newenvironment{Discuss}{\begin{large}\begin{em}**********
    things to be discussed ********** \\}{\\ **********\end{em}\end{large}}
% set the paragraph identation and separation


% the foil environment
\newenvironment{Foil}{\begin{document}\begin{LARGE}\begin{sf}
    }{\end{sf}\end{LARGE}\end{document}}
    % NOTE: ``}'' must be in the 2nd line
% foil page title
\newcommand{\Title}[1]{\newpage \center{\huge {\sf #1}} \flushleft
    \vspace{1ex}}

% set the paragraph identation and separation
\parindent 0.2in
\setlength{\parskip}{1ex}

% set text width
\textwidth = 6.75in

% set the formula separation
\setlength{\topsep}{0in}

% set indentation for formulas:
% \setlength{\mathindent}{3ex}

% set left margin
\setlength{\oddsidemargin}{-.1in}




==> arXiv - Copy/model.tex <==
%auto-ignore
\section{Long Short Term Memory Enhanced Spatio-Temporal Point Process}\label{sec:model}

Equation~(\ref{density}) shows that traditional TPP models depend conditionally on $H$, the time of historical events. Let $u$ and $l$ denote the user and location of interest, respectively (an event being $u$ check-in to $l$). As we discussed before, such historical events are scarce in check-in data due to the lack of repeated check-ins to the same location by a user. This causes difficulties in both training and predicting stage of TPP models. We propose to enrich the event sequences with \textit{Precedent Check-ins}, which are check-ins a user reported before check-in to $l$ on his/her trajectory. Figure~\ref{sequence} illustrates a normal sequence of events and the same sequence enriched with precedent check-ins.

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.40]{sequence.pdf}
\end{center}
\caption{Example of an enriched event sequence. }\label{sequence}
%\vspace{-7mm}
\end{figure}

Recall the previous example of visiting restaurants and shops. If a user check-ins to a restaurant, this behaviour shall decrease the user's intensity to visit another restaurant at the moment. But check-in to a shop may not effect the intensity to visit a nearby shop of the same type. Similarly, moving towards or away from a location shall cause the intensity to visit the location to fluctuate accordingly. These examples are only to demonstrate the possible influence of precedent check-ins on the intensity function. The actual dependency could be much more complex, for which we will have the LSTM-STPP model to discover from the check-in data.


\subsection{Feature Representation}

Before we feed an enriched event sequence to our model, each check-in in the sequence needs to be represented as a feature vector, which contains the information about the check-in in a structured manner. The feature vector for a check-in $c_i$ is denoted by $\boldsymbol{y_i}$, which consists of the following elements:

\begin{enumerate}[leftmargin=*]
\item Localized event time $t_i \in \mathbb{R}$. Time of the earliest check-in to the location is set to 0 and the rest times are set accordingly in the unit of hours or days.

\item Additional time-date information which indicates if the check-in occurred in a weekday or a weekend, and in what time period of the day (e.g., morning, afternoon, or midnight). This is because human demonstrates different check-in patterns in different time periods.

\item Euclidean distance of the check-in location to the location of interest $l$. The distance is computed using coordinates of the locations and normalized to the range of $[0,1]$, where $1$ indicates the distance is negligible, while $0$ means the distance is larger than a distance threshold denoted by $\theta_D$. 

\item Category of the check-in location, such as \textit{Restaurant, Hotel, Bar,} etc. We use a $x$-dimension value to represent the category information where $x$ is the total number of location categories. The $i$-th element is set to $1$ if the location belongs to the $i$-th category, otherwise $0$.

\item User overlapping with the location of interest $l$. Let $p$ denote the check-in location of $c_i$. We compute the proportion of users that have visited both $p$ and $l$ within a given time window. It reflects the inherent relevance of the two locations. The overlapping ratio is computed as follows:
\begin{align}
OR = C_{l,p}^v \Big/ \sqrt{C_l^v C_p^v},
\end{align}
where $C_{l,p}^v$ is the number of users who visited both $l$ and $p$ within a time window $v$. $C_l^v$ and $C_p^v$ are the number of visitors to $l$ and $p$ within the time window, respectively.

\item Previous check-in by friends, which reflects the social aspect of check-in behaviors. We calculate the minimal time interval from $t_i$ to a check-in to the location of interest by a friend of the user. The value is normalized such that $1$ indicates a friend just check-in to the location, while $0$ means the minimal time interval is larger than a threshold denoted by $\theta_T$.

\end{enumerate}

Each vector is also associated with a Boolean value indicating if it is an event or a precedent check-in. Unfortunately, not all the above information are always available on LBSNs. e.g., some LBSNs hide user's social connections, or do not provide location categories. In such cases the unavailable features are ignored in generating the vector. Therefore, the total dimension of the feature vector may vary depending on the specific data source. Comparing with $\boldsymbol{y_i}$, the user feature vector $\boldsymbol{p_u}$ is simpler. It contains two elements. 

The first element is the user's preference to the location of interest $l$. We incorporate both explicit and implicit preference. Explicit preference is the user's rating for $l$, which is usually not directly available for every location, but can be estimated using techniques such as matrix factorization~\cite{koren2009matrix}. As for implicit preference, we calculate the user's check-in frequency to $l$, i.e., the total number of check-ins to $l$ on the user's trajectory, divided by the length (time between the first and the last check-in) of the trajectory.

The second element is the user's homebase, i.e., the center and range of the user's daily movements. The explicit homebase are usually unknown. Here we use the method introduced in~\cite{yang2016spatio} to estimate a user's homebase using the distribution of his historical check-ins. We then use the normalized distance from the estimated homebase to the location of interest as the feature value.


\subsection{Model Architecture}

Figure~\ref{RNN} gives a high-level illustration of the proposed model, which consists of an input layer, an output layer, several hidden layers, and inner weight matrices that store weights on the edges. 

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.55]{RNN.pdf}
\end{center}
\caption{LSTM-STPP model architecture.}\label{RNN}
%\vspace{-7mm}
\end{figure}

The input to the model is a sequence of events enriched with precedent check-ins, denoted by $\{ c_1, c_2, ..., c_n \}$ where $c_i$ $(1 \leq i \leq n-1)$ can be either an event or a precedent check-in. Using these check-ins, we want to predict the next event time after $C_n$. When feed into the model, a check-in $c_i$ is represented by a feature vector $\boldsymbol{y_i}$. The model then iterates through the input sequence in $n$ steps, and updates its status at each step.

We now discuss how to update the internal status of the neural network. The internal status of the model at the $i$-th step can be represented as a vector $\boldsymbol{h_i}$. In each step, the vector which is updated by several hidden neural network layers according to the previous network status and current inputs. The location information of check-ins is incorporated into the status vector during this updating process, which we illustrate in Figure~\ref{}.

The first step of status updating is to discard, or ``forget" irrelevant information from historical events. This is implemented by the forget gate layer $\boldsymbol{ F_t }$, which is computed as follows in our model:
\begin{align}
\boldsymbol{ F_t } = 	\begin{cases} 
		g( \boldsymbol{ M_F } *[ \boldsymbol{ h_{i-1}, Y_i }  ] + b_F), & \text{if } c_i \text{is an event} \\
		1 & \text{otherwise} 
		\end{cases}
\end{align}
Here, $\boldsymbol{ M_f }$ is the weight matrix of the forget gate layer, $b_F$ is a constant, and $g(\cdot)$ is an activation function, for which we choose the sigmoid function $g(x) = exp(1/1+e^{-x})$. $[ \cdot, \cdot]$ denotes the concatenation of two vectors. And finally, $\boldsymbol{Y_i}$ is the accumulated check-in information from successive check-ins occurred in a certain time window $w$, which is defined as follows:
\begin{align}
\boldsymbol{ Y_i } = \sum_{(t_i - t_j < w)} \boldsymbol{ M_{t_i - t_j} * y_j }
\end{align}
where the condition $t_i - t_j < w$ defines a time window that includes all the precedent check-ins and events within $w$ from the time of $c_i$ (including $c_i$). The time window $w$ can be further partitioned into several intervals, and $M_{t_i - t_j}$ is a transition matrix specifically for the internal that covers $t_i - t_j$.  This term is meant to capture the influence of recent precedent check-ins in different time windows that may lead to the current event.

Then, the model decides which new information shall be stored, this is implemented with two separated neural network layers, the input gate layer $ \boldsymbol{I_i}
$ and the candidate cell status layer $\boldsymbol{\tilde{S}_i}$. We have the following updating functions:
\begin{align}
\boldsymbol{I_i} = \begin{cases}
	   g( \boldsymbol{ M_I } * [ \boldsymbol{ h_{i-1}, Y_i }  ] + b_I ), & \text{if } c_i \text{is an event} \\
	   g( \boldsymbol{ M_I'} * [ \boldsymbol{ h_{i-1}, y_i } ] + b_I' ), & \text{otherwise} 
	   \end{cases}   
\end{align}

\begin{align}
\boldsymbol{\tilde{S}_i} = \begin{cases}
	   			h( \boldsymbol{ M_S } [ \boldsymbol{ h_{i-1}, Y_i}  ] + b_S), & \text{if } c_i \text{is an event} \\
	  			h( \boldsymbol{ M_S' } [ \boldsymbol{ h_{i-1}, y_i} ] + b_S'), & \text{otherwise} 
	   		   \end{cases}
\end{align}
In the above equations, $\boldsymbol{M_I, M_I', M_S, M_S'}$ are weight matrices and $b_I,b_I',b_S,b_S'$ are constant parameters. $h$ is another activation function which we use $tanh(\cdot)$ since we want the output value to be in the range of $[-1,1]$.

The next step is to update the cell status, denoted by $\boldsymbol{S_i}$. It is updated by ``forget" the information marked by the forget gate layer while ``remember" new information provided by the input gate and candidate status layer:
\begin{align}
\boldsymbol{S_i} = \boldsymbol{ F_t S_{i-1}} + \boldsymbol{ I_i \tilde{S}_i}
\end{align}
After the updating, the cell status now records the information that should be passed to the next step. And finally, we can update the vector representation of the  internal network status:
\begin{align}
\boldsymbol{h_i} = \begin{cases}
	   g( \boldsymbol{ M_H } [ \boldsymbol{ h_{i-1}, Y_i}  ] + b_H) h(\boldsymbol{S_i}), & \text{if } c_i \text{is an event} \\
	   g( \boldsymbol{ M_H' } [ \boldsymbol{ h_{i-1}, y_i} ] + b_H') h(\boldsymbol{S_i}), & \text{otherwise}
	  \end{cases}   
\end{align}
Note that both $\boldsymbol{S_i}$ and $\boldsymbol{h_i}$ are passed to the next step of the model, thus an recurrent status update is implemented.

Intuitively, the status vector $\boldsymbol{h_i}$ can be seen as a latent representation of knowledge learned from all previous check-ins by the model. We can now compute the conditional density function of next event time using $\boldsymbol{h_i}$ as follows:
\begin{align}
\lambda(t) = exp \Big( \boldsymbol{W}^T \boldsymbol{ h_i} + \beta_t (t-t_i) + \beta_d D + \boldsymbol{B}^T \boldsymbol{p_u} + b \Big)
\end{align}
The computation involves several factors: $\boldsymbol{W}^T \boldsymbol{ h_i}$ computes the influence of previous check-ins, $\beta_t (t-t_i)$ and $\beta_d d$ represent current temporal and spatial impact, respectively, and $D$ is the Euclidean distance between current location and the location of interest. The vector $\boldsymbol{p_u}$ represents information of the user, which allows the function to be personalized for a given user $u$. Finally, $b$ is a constant base intensity for the location. Note that the exponential function guarantees the intensity is positive.

The intensity function is then used to predict the time interval between current check-in $c_i$ and the next event $c_j$:
\begin{align}
\hat{I}_{i,j} = \hat{t}_{j} - t_i,
\end{align}
where $\hat{t}_{j}$ is estimated using Equation~(\ref{expect}). The predicted value $\hat{I}_{i,j}$ is the only output of the model at each step. 

Note that the LSTM-STPP model may generate multiple predictions for the time of the same event. This is because if an event has precedent check-ins, each of the check-ins will generate an output but they have the same next-event. In this case, we will use the output of the most recent precedent check-in as the final prediction for the event time. There are two reasons behind this: First, temporally close check-ins are usually more relevant to each other. Second: The output of the most recent precedent check-in is supposed to incorporate information of all the precedent check-ins and historical events, thus shall contain more complete information. If an event has no direct precedent check-ins, i.e., it is preceded by another event with no other check-in in between, then the event will have a single predicted time. This design guarantees that a valid prediction can be made even for users who have never visited the location of interest. In that case, all his/her check-ins will be treated as precedent check-ins, and no event is included in the sequence.

% Multiple predictions for the same time point...

\subsection{Model Training}

For a given location of interest, the training dataset is a collection of historical user trajectories. Each trajectory contains at least one check-in to the location as ground truth. We use the classic Back Propagation Through Time~\cite{rumelhart1988learning} for LSTM networks to train the proposed RSTPP model. We use the cycle unrolling technique and unroll the recurrent neural network by $s$ steps. The model parameters are shared among the unrolled copies of the neural network. Similarly, the training sequences are also partitioned into batches of subsequence which contains at least $s$ consecutive check-ins. The loss function we used is the negative log-likelihood of observing the training instances (given in Equation~\ref{MLE}). In each iteration of the training process, output of the model is feed into the loss function and its parameters are updated accordingly in the back propagation stage using stochastic gradient descent until achieve convergence.

==> arXiv - Copy/problem.tex <==
%auto-ignore
\section{Problem Formulation} \label{sec:problem}

\subsection{Threat Model}

\myparatight{Attack goal} We consider an attacker's goal is to \emph{promote} a target item $t$ to as many users as possible. %Suppose the recommender system has $|U|$ users $U = \{ {u_1},{u_2},...,{u_{|U|}}\}$ and $|I|$ items $I = \{ {i_1},{i_2},...,{i_{|I|}}\}$. 
Suppose the system recommends $N$ items to each user. We denote by $h(t)$ the fraction of normal users whose top-$N$ recommendations include the target item after the attack. $h(t)$ is called \emph{hit ratio} of the target item $t$. The attacker's goal is to maximize the hit ratio. We note that an attacker could also \emph{demote} a target item, i.e., minimize the hit ratio of the target item. However, demotion is a special case of promotion~\cite{mobasher2007toward,yang2017fake}. Specifically, an attacker can promote other items such that the target item is demoted in recommendation lists. Therefore, we will focus on promotion attacks in this work.  


%Supposes there are $|U|$ users $U = \{ {u_1},{u_2},...,{u_{|U|}}\}$ and $|I|$ items $I = \{ {i_1},{i_2},...,{i_{|I|}}\}$ in a recommender system. Let $R \in {{\mathbb{R}}^{|U| \times |I|}}$ denote the rating matrix, $r_{ui}$ is the rating of user $u$ on item $i$, and $t \in I$ the target item selected by the attacker. The goal of attack is to promote the target item by spoofing the recommender system. i.e., making the target item to appear in the top-$N$ recommendation list of as many normal users as possible.


\myparatight{Attack approach} The attacker uses data poisoning attacks to achieve the attack goal. In particular, the attacker injects some fake users to the system. Each fake user gives a high rating score to the target item and well-crafted rating scores to certain selected items, which we call \emph{filler items}. A key challenge for the attacker is to determine the filler items and their rating scores for each fake user. Since normal users often rate a small number of items, we assume the number of filler items for each fake user is at most $n$, to avoid being detected simply based on the number of rated items. 

%are realized by injecting a set of fake accounts into the system. We will refer to these injected fake accounts as fake users. Each fake user will give a fake rating to the target item, along with certain fake ratings to a set of carefully selected filler items, denoted by ${I_F}$. The filler items are meant to hide the fake rating to the target item among some other items to make it less obvious. These fake ratings are designed to cause the system to have a bias toward the target item $t$, making it more favorable when generating recommendations to normal users.

\myparatight{Attacker's background knowledge and capability} We assume an attacker has the following background knowledge: 1) the recommendation algorithm used by the given recommender system; and 2) the user-item rating score matrix, which is usually publicly available and can be collected by the attacker. We note that the attacker could also collect a partial  user-item rating score matrix for a subset of users and subset of items, and design attacks based on the partial matrix. Our threat model is also known as \emph{white-box} setting. In our experiments, we will demonstrate that our attacks can also be transferred between recommender systems under the \emph{grey-box} setting (i.e., the attacker does not know the parameters of the recommendation algorithm) or the \emph{black-box} setting (i.e., the attacker does not know the recommendation algorithm). 

In practice, an attacker often has limited resources so the attacker can only inject a bounded number of fake users into the system, though the bounded number could still be large. For instance, an attacker could leverage compromised machines to register and maintain fake users. Detecting such fake users is also known as \emph{Sybil detection}, and many methods (e.g.,~\cite{Wang13Clickstream,EVILCOHORTSecurity15,sybilbelief}) have been developed to detect fake users. For instance, the service provider could analyze the IP addresses of the users to detect fake ones. To avoid such IP-based detection, 
an attacker often registers a small number of fake users on a compromised machine. Indeed, Thomas et al.~\cite{SybilUnderground13} found that a half of compromised machines under an attacker's control maintain less than 10 fake users in online social networks. %The service provider could also extract features from An attacker could 
More formally, we assume the attacker can inject $m$ fake users into the recommender system. 

%For instance, if the attacker injects too many fake users, it may be easier for the recommender system to detect them. 


%The service provider could leverage  machine learning techniques to detect fake users. In fact, detecting such fake users is also known as \emph{Sybil detection} and many methods have been developed to detect 
%
%To avoid being detected (e.g., the service provider could analyze IP addresses of users to detect fake users), an attacker often registers a small number of fake users on a compromised machine. Indeed, in the domain of social media, Thomas et al.~\cite{SybilUnderground13} found that a half of compromised machines under an attacker's control maintain less than 10 fake users. 
%
%
%We assume the attacker has limited resources such that the attacker can only inject $m$ fake users into the system. For instance, if the attacker injects too many fake users, it may be easier for the recommender system to detect them. 



% 3) The attacker has the ability to inject fake accounts into the system, e.g., register users with fake profile using the registration system.
%
%We also assume the attacker has limited resources so it can inject only a limited number of fake accounts. Otherwise, the attacker can flood the system with unlimited number of fake accounts and trivially manipulate any recommendation result as he desires.
%
%In order to launch a successful shilling attack, three key questions must be answered:
%\begin{itemize}
%\item \textbf{First, how to select the filler items?} The item set commonly contains millions of items. We want to select a small set of filler items through which the target item can be promoted in the most efficient way.
%\item \textbf{Second, how many fake accounts should be injected?} Injecting more fake accounts is likely to have more impact on the target item. However, the dilemma is that a larger number of fake accounts are usually much easier to be detected~\cite{mehta2009unsupervised}.
%\item \textbf{Third, how to determine which filler item(s) should be rated by each fake account?} Finding the optimal combination of fake accounts and filler items is not trivial. This is because the distribution of ratings from the fake accounts should mimic the behavior of normal users (who typically rate only a small fraction of items) to avoid being easily detected, while still try to maximize the positive impact on the target item.
%\end{itemize}
%Our research aims to answer the above questions in a systematic way.


\subsection{Attacks as an Optimization Problem}

%We are interested in finding an optimal attacking strategy, which can achieve the maximal attacking outcomes with a limited number of fake users. 

We formulate poisoning attacks as an optimization problem, solving which maximizes the hit ratio of the target item. % and explore its solution space to find the best attacking strategy. 
Let $r_v$ be the rating score vector of a fake user $v$, where $r_{vi}$ is the rating score that the fake user $v$ gives to the item $i$. We consider a rating score is in the set of integers $\{0, 1, \cdots, r_{max}\}$, where $r_{max}$ is the maximum rating score. For instance, in many recommender systems, $r_{max}=5$. A rating score of 0 means that the user did not rate the corresponding item. Essentially, we aim to find the rating score vector for each fake user that maximizes the hit ratio of the target item. Specifically, we find the rating score vectors via solving the following optimization problem:
\begin{align}
\label{objectiveFrame}
\text{max }  &  h(t)    \\
%\label{budgetconstraint}
\text{subject to } & |r_v|_0 \leq n + 1, \forall v\in \{v_1, v_2, \cdots, v_m\}  \nonumber \\
%\label{itemRating}
& r_{vi} \in \{0,1,\cdots,r_{max}\},  \forall v\in \{v_1, v_2, \cdots, v_m\}, \nonumber
\end{align}
where $\{v_1, v_2, \cdots, v_m\}$ is the set of $m$ fake users, $|r_v|_0$ is the number of non-zero entries in the rating score vector $r_v$, and $n$ is the maximum number of filler items (the filler items do not include the target item). The hit ratio $h(t)$, which is the fraction of normal users whose top-$N$ recommended items include the target item $t$, is computed by a  recommender system on the entire user-item rating score matrix that includes the $m$ fake users. We note that our formulation in Equation~\ref{objectiveFrame} is applicable to data poisoning attacks to any recommender system. In this work, we will focus on graph-based recommender systems. 



%Let $m$ denote the maximum number of fake users that can be injected into the system, and each fake user is allowed to show his/her preference on at most $n$ items. We will use $V = \{ v_1, v_2, ... v_m \}$ to denote the set of fake users. These users are injected to the system one-by-one and $v_i$ denotes the $i$-th injected fake user. Each fake user $v_i$ will submit fate ratings to the target item $t$ and his/her filler items. These filler items are selected from a candidate item set, denoted by $C$, where $C \triangleq I\backslash \{ t\}$. Formally, we define variable ${\mathds{1}_{{v_i}}}\left( j \right)$ as a indicator of whether or not fake user ${v_i}$ selects item $j$ as one of the filler items:
%\begin{align}
%{\mathds{1}_{{v_i}}}\left( j \right) \triangleq \begin{cases}	
%	1, & \mbox{if fake user $v_i$ select item $j$ as filler item,}\\
%	0, & \mbox{otherwise,}	
%\end{cases}
%\end{align}
%where ${v_i} \in V$, $j \in C$ and $1 \le i \le m$. Let ${I_F}({v_i})$ denote the filler items selected by fake user ${{v_i}}$. After we use certain rating strategy to rate each of these filler items and the target item, we inject the attack profile of fake user $v_i$, ${S_{{v_i}}}$ into the system.
%
%Let ${\ell _u}\left( {{S_v}} \right)$ be the set of top-$N$ recommendations for normal user $u$ \textit{after} injecting $m$ attack profiles into the recommender system. Since our goal is to make the target item to be recommended to as many normal users as possible, we purpose a straightforward metric called \textit{hit ratio} (${h_u}\left( t \right)$) to measure the attack outcome. \textit{Hit Ratio} (\textbf{HR}) reflects whether or not the target item $t$ appears in ${\ell _u}\left( {{S_v}} \right)$, which is computed as:
%\begin{align}
%{h_u}\left( t \right) \triangleq \begin{cases}
%1, & \mbox{if $t \in {\ell _u}\left( {{S_v}} \right)$},\\
%0, & \mbox{otherwise}.
%\end{cases}
%\end{align}
%Our goal is to maximize the hit ratio of the target item $t$, under the constraint that as most $m$ attack profiles can be injected. We formulate this problem as the following optimization problem:
%\begin{align}
%\label{objectiveFrame}
%\text{Maximize}  & \ \textstyle \frac{1}{{\left| U \right|}}\sum\limits_{u \in U} {{h_u}\left( t \right)}  &  \\
%\label{budgetconstraint}
%\text{s.t. } & \textstyle \sum\limits_{j \in C} {{\mathds{1}_{{v_i}}}\left( j \right)}  \le n,\  & 1 \le i \le m,  \forall j \in C, &  \\
%\label{itemSelected}
%& {\mathds{1}_{{v_i}}}\left( j \right) \in \{0, 1\},\  & 1 \le i \le m, \forall j \in C, & \\
%\label{itemRating}
%& r({\mathds{1}_{{v_i}}}\left( j \right)) \in [{r_{\min }},{r_{\max }}], &1 \le i \le m, \forall j \in {I_F}({v_i}),
%\end{align}
%where $r({\mathds{1}_{{v_i}}}\left( j \right))$ is the rating fake user $v_i$ give to its filler item $j$, ${r_{\min }}$ is the minimum rating and ${r_{\max}}$ is the maximum rating. Intuitively, in our formulation, Equation~(\ref{objectiveFrame}) indicates that the attacker aims to maximize the HR; Equation~(\ref{budgetconstraint}) and  Equation~(\ref{itemSelected}) guarantee that no more than $m$ fake users can be injected into the system, and each fake user is allowed to rate at most $n$ items. Equation~(\ref{itemRating}) guarantees that fake user $v_i$ rate each filler item $j \in {I_F}({v_i})$ with a value between ${r_{\min }}$ and ${r_{\max}}$. The above optimization problem relies on a set of integer variables. Such integer optimization problems are known to be intractable thus finding optimal solutions can be challenging for an attacker with limited resources. Accordingly, in the next section, we shall develop heuristic, a supervised random walk based attack algorithm which relaxes some of the constraints and hence makes the problem tractable. Specifically, we inject fake accounts one-by-one into the system and ensure that each fake user achieves the optimal attack impact by considering the impact of previously injected fake accounts. Our attack algorithm enjoys low-complexity and more importantly, we show that even using such sub-optimal attacking strategies, our attack can make significant impact with a relatively small attack size, i.e., the ratio between the number of injected fake users and the population of normal users in the system.



==> arXiv - Copy/related.tex <==
%auto-ignore
\section{Background and Related Work} \label{sec:related}

\subsection{Collaborative Filtering}
Collaborative filtering based recommender systems have been widely deployed in various web services such as Amazon, YouTube, Netflix, and Google Play. Suppose we are given a \emph{user-item rating score matrix}, where the entry $r_{ui}$ is the rating score that user $u$ gave to item $i$, e.g., a product on Amazon, a video on YouTube, a movie on Netflix, and an app on Google Play. For instance, a rating score $r_{ui}$ can be 0, 1, 2, 3, 4, or 5, where $r_{ui}$=0 indicates that $u$ did not rate the item $i$, 1 means the most negative rating score, and 5 means the most positive rating score. The goal of collaborative filtering is to recommend \emph{each} user in the user-item rating score matrix $N$ items that the user did not rate before but the user may have interests in, via analyzing the rating score matrix. Depending on the techniques that are used to analyze the rating score matrix, collaborative filtering can be roughly classified to 4 categories, i.e., \emph{neighborhood-based}, \emph{association-rule-based}, \emph{matrix-factorization-based}, and \emph{graph-based}. 

\myparatight{Neighborhood-based, association-rule-based, and matrix-fac-torization-based recommender systems}
Neighborhood-based recommender systems~\cite{sarwar2001item} find neighbors of a user or neighbors of an item in order to recommend items to a user. For instance, to recommend a user items, the methods  can first find the nearest-neighbors of the user, predict the user's rating scores to items based on the rating scores of the nearest neighbors, and recommend the $N$ items that have the highest predicted rating scores to the user. 
%then user $u$ gets recommendations to items that are already positively rated by users in his/her neighborhood.
Association-rule-based recommender systems~\cite{mobasher2000automatic,davidson2010youtube} aim to identify frequent co-occurrence between items in user reviews. For instance, if many users give high rating scores to both item $A$ and item $B$, then there is a certain association between the two items. For a user who gave a high rating score to item $A$, item $B$ is recommended to the user. %Likewise, on YouTube, if two videos are watched together by many users, then the two videos have a certain 
Matrix-factorization-based recommender systems~\cite{MFRec09} assume that the user-item rating score matrix can be explained by a small number of latent factors. Based on the assumption, they use a low-rank matrix to approximate the user-item rating score matrix. The low-rank matrix predicts missing values in the user-item rating score matrix, i.e., for each user, the low-rank matrix predicts rating scores to all items that the user did not rate before; and the $N$ items that have the highest predicted rating scores are recommended to the user.  



%\noindent
%{\bf Association-rule-based.} Association rule captures the relationships between items based on their patterns of co-occurrence in
%many transactions~\cite{mobasher2000automatic}. Here, a transaction is a set of items that have been rated by a user over a period of time. An example of an association rule is that 90\% of the people watch Gone with the Wind and The Bridges of Madison County in a given month, also watch Titanic later. In a association rule based collaborative filtering, it first build a prediction model based on all significant association rules, then recommend to users the top-$N$ items that are associated with the items that they have already rated.


%\noindent
%{\bf Matrix-factorization-based.} Matrix factorization~\cite{MFRec09} is one of the most popular recommendation algorithms. MF maps users and items into a latent factor of $d$-dimensional space, user $u$ is represented by a latent vector $x_u \in {{\mathbb{R}}^{d}}$ and item $i$ by a latent factor $y_i \in {{\mathbb{R}}^{d}}$. A rating predicted by user $u$ to item $i$ is given by
%\begin{align}
%\hat{r}_{ui} = \mu  + {b_i} + {b_u} + y_i^T{x_u},
%\end{align}
%where $\mu$ is the total average of all ratings, $b_u$ and $b_i$ are the user and item biases respectively. We can learn the parameters ($b_u$, $b_i$, $x_u$ and $y_i$) by minimizing the following objective function:
%\begin{align}
%\mathop {\min }\limits_{{x^*},{y^*},{b^*}} {\sum\limits_{u,i} {({r_{ui}} -\hat{r}_{ui})} ^2} + \eta (||{x_u}|{|^2} + ||{y_i}|{|^2} + ||{b_u}|{|^2} + ||{b_i}|{|^2}),
%\end{align}
%where $\eta$ is the regularization parameter. Although MF is effective in making good recommendations, it is also known to suffer from the cold start problem~\cite{MFRec09}, i.e., it is challenging to generate high-quality recommendations for users who have little item rating/visiting history.





%A recommender system takes as input a set of users and a set of items (e.g., products on Amazon, videos on YouTube), and find a subset of items that are most likely to be preferred by a given user. Based on the their techniques, existing recommender systems generally fall in two categories, \textit{content-based} systems \cite{contentbasedLang95,contentbasedPazzani97} and \textit{collaborative filtering} based systems~\cite{userUserRec94,amazonRecommendation,davidson2010youtube,MFRec09,LiuWSDM15,LiuTKDD16}. The major difference is that content-based systems make recommendations by extracting descriptive information from the content of items, while collaborative filtering systems focus on exploring the inherent similarity between items and users, i.e., items recommended to a user are usually those preferred by similar users. There are also several techniques~\cite{melville2002content,lu2015content} that attempt to combine the two types of techniques to make more accurate recommendations.
%
%Content-based recommendation requires the system to ``understand" the content of items, which usually relies on human labor and/or machine learning techniques such as Natural Language Process. In contrast, collaborative filtering only requires the knowledge of historical visits to the items, i.e., which user has visited (e.g., viewed, purchased, rated) which items, thus it is usually considered easier to deploy on large scale. Interested readers are referred to surveys~\cite{RecSurveyTKDE05,RecSysSurvey13} for detailed explanation and comparisons of different types of recommender systems.

\myparatight{Graph-based recommender systems} In this work, we focus on graph-based recommender systems~\cite{fouss2007random}. Graph-based recommender systems were deployed by several popular web services such as eBay~\cite{eBay2013a,eBay2013b} and Huawei App Store~\cite{He15,Guo17} in China. %Such systems also demonstrated excellent performance on various recommendation tasks including tag recommendation~\cite{guan2009personalized} and image retrieval~\cite{xu2011efficient}. In this paper, we present a systematic study of shilling attack targeting graph-based recommender systems.
 The key idea of graph-based recommender system is to model users' preference for items as a weighted bipartite graph $G =  ( U, I, E )$, namely \emph{user preference graph}. The two sets of vertex $U$ and $I$ represent the user set and the item set, respectively;  an edge $(u,i)$ between a user $u \in U$ and an item $i \in I$ represents that the user rated the item; and the  weight of an edge $(u,i)$ is the rating score that the user gave to the item.  
%The absence of an edge $(u, i)$ indicates user $u$ has not rated item $i$ thus his preference for the item is unknown. 
Figure~\ref{graph-based} illustrates a user preference graph with an example of 3 users and 3 items. %In this case, the weight on an edge is in proportion to a user's explicit rating to a specific item.

\begin{figure}[!t]
	\centering
	\includegraphics[scale = 0.55]{figs/fig1.pdf}
	\caption{An illustration of user preference graph}\label{graph-based}
\end{figure}

To generate the top-$N$ recommendation list for a user, the recommender system performs a \emph{random walk} in the graph, where the random walk starts from the user and jumps back to the user with a probability $\alpha$ in each step, where $\alpha$ is called \emph{restart probability}. The stationary probability distribution of the random walk is used to rank items and make recommendations. We denote by $p_u$ the stationary probability distribution of the random walk that starts from the user $u$. Then, the stationary probability distribution is a solution of the following linear system:
\begin{align}
\label{RWR}
p_u = (1 - \alpha ) \cdot Q \cdot p_u + \alpha  \cdot e_u,
\end{align}
where $e_u$ is a unit vector whose $u$th entry is 1 and all other entries are 0, and the matrix $Q$ is called \emph{transition matrix}, which is defined as follows:
\begin{align}
\label{matrixQ}
{Q_{xy}} = \begin{cases}
\frac{{{r_{xy}}}}{{\sum\limits_{z \in {\Gamma_x}} {{r_{xz}}} }} & \mbox{if $(x, y) \in E$}\\
0 & \mbox{otherwise,}
\end{cases}
\end{align}
where $\Gamma_x$ is the set of neighbors of node $x$. More specifically, for a user node $x$, $\Gamma_x$ is the set of items that were rated by $x$; for an item node $x$, $\Gamma_x$ is the set of users that rated $x$.
To solve $p_u$, we start from a random probability distribution and then iteratively update $p_u$ as $p_u^{(t+1)} = (1 - \alpha ) \cdot Q \cdot p_u^{(t)} + \alpha  \cdot e_u$ until convergence. Then, we rank the items that were not rated by the user $u$ with respect to their stationary probabilities. The top-$N$ items with the largest stationary probabilities are recommended to the user $u$. 


%from the user preference graph. Specifically, the items that are most likely to appear on the random walk path originate from a user $u$ are used as candidates for the user's top-$N$ recommendation list. The logic behind this recommendation is that such items are likely to be similar to the ones that $u$ already likes. Given a preference graph, several types of random walk-based recommendation algorithms were proposed, due to limited space, reader are referred to~\cite{fouss2007random,pham2015general} for a details of these algorithms.


\subsection{Attacks to Recommender Systems}

%Two types of attacks to recommender systems have been studied in the literature. \textit{Security Attacks} aim to spoof a recommender system to make recommendations as the attacker desires, i.e., promote a target item. The goal of \textit{Privacy Attacks} is to infer private information about a user by analysis the recommendation results. We briefly summaries representative works on these two types of attacks.

\subsubsection{Security Attacks} These attacks aim to spoof a recommender system such that a target item is recommended to as many or few users as possible.  Specifically, \emph{poisoning attacks} (also known as \emph{shilling attacks})~\cite{profileinjectionattacksMahony04,lam2004shilling,mobasher2007toward} aim to inject fake users with fake rating scores to the system such that a bad recommender system is learnt from the user-item rating score matrix. \emph{Profile pollution attacks}~\cite{xing2013take} aim to pollute the rating behavior of normal users to manipulate the recommendations to them. By analogy to adversarial machine learning,  poisoning attacks are to manipulate recommender systems at ``training time", while profile pollution attacks are to manipulate recommender systems at ``testing time". 



\myparatight{Poisoning attacks}   Poisoning attacks were first studied more than a decade ago~\cite{profileinjectionattacksMahony04,lam2004shilling,mobasher2007toward}. However, these attacks are heuristics-driven and are not optimized to a particular type of recommender systems. For instance, in \emph{random attacks}~\cite{lam2004shilling}, given the number of fake users an attacker can inject into the system, the attacker randomly selects some items for each fake user and then generates a rating score for each selected item from a normal distribution, whose mean and variance are calculated from the rating scores in the entire user-item rating score matrix. In \emph{average attacks}~\cite{lam2004shilling}, the attacker generates a rating score for a selected item from a normal distribution, whose mean and variance are computed from the rating scores to the selected item in the user-item rating score matrix. 

More recent poisoning attacks~\cite{poisoningattackRecSys16,yang2017fake} generate fake rating scores or behavior that are optimized to a particular type of recommender systems.  Specifically, Li et al.~\cite{poisoningattackRecSys16} proposed poisoning attacks to matrix-factorization-based recommender systems. Yang et al.~\cite{yang2017fake} proposed poisoning attacks (they called them \emph{fake co-visitation injection attacks}) to association-rule-based recommender systems, in which each user injects fake co-visitations between items instead of fake rating scores to items.  We aim to study optimized  poisoning attacks to graph-based recommender systems. 

%In a very recent work~\cite{yang2017fake}, Yang et al. proposed fake co-visitation injection attack which targets co-visitation based recommender systems. This attack leverages a data structure namely co-visitation graph which records how many times two items have been co-visited by the same set of users. By forging co-visitations between selected items, their attack can successfully promote or demote a target item. Fake co-visitation injection attack does not rely on CSRF since it does not spoof user-profiles to achieve the attack goal. However, this attack requires the attacker to have knowledge about the items as well as their co-visitations, which is usually not available in reality. Without such knowledge, launching attacks would require a much higher cost and thus make the attack easier to be detected.
%
%
%There are several studies~\cite{profileinjectionattacksMahony04,lam2004shilling,mobasher2007toward} revealed that \emph{user-item rating matrix}-based recommender systems (e.g., \cite{userUserRec94,amazonRecommendation,MFRec09}) are vulnerable to \emph{shilling attacks}. Specifically, in a user-item rating matrix, each row corresponds to a registered user and each column corresponds to an item; an entry in the matrix is the rating score that the corresponding user give to the corresponding item; a rating score represents the corresponding user's preference to the corresponding item. Most entries of the matrix are missing since a user usually only provides feedback to a small number of items. Such recommender systems attempt to infer the missing values in the matrix and make recommendations based on these values. In a shilling attack, an attacker first registers a large number of fake accounts in the service. Then each fake account gives certain rating scores to a carefully chosen subset of items. As such, shilling attack is also referred to as \emph{profile injection attack}. 
%
%In response to shilling attack, several techniques have been proposed for detection of injected fake accounts~\cite{burke2006classification}. It has been shown in these studies that the more fake accounts an attacker injects, the easier it is to detect them. Consequently, applying shilling attack on large scale in return makes them much easier to be detected. To circumvent this problem, some shilling attacks proposed to leverage a small set of existing seed users who are influential, instead of injecting fake accounts. However, acquiring seed users' cooperation is not trivial in reality. In this paper, we propose to advance this line of research with a novel optimization framework for shilling attacks, which does not suffer from the above limitations.




\myparatight{Profile pollution attacks} Xing et al.~\cite{xing2013take} proposed {profile pollution attacks} to recommender systems and other personalized services, e.g., web search. Their attacks aim to pollute a user's profile, e.g., browsing history, via cross-site request forgery (CSRF)~\cite{CSRF}. With a polluted user profile, the attacker can recommend arbitrary items to the user. 
They showed that  popular web services including YouTube, Amazon, and Google search are vulnerable to the attacks. However, the limitation of these attacks is that they rely on CSRF, which makes it hard to perform the attacks at a large scale.

%Pollution attack aims to make a target item to appear in the recommendation result to a specific victim user, which is achieved by injecting fake information (e.g., fake clicks, fake rating) into the victim user's profile (e.g., browsing history). The attack relies on cross-site request forgery (CSRF)~\cite{CSRF} to inject such fake information. Pollution attacks represent the first step towards attacking user-to-item recommendation. However, 
%it has two key limitations: 1) pollution attacks rely on CSRF, which makes it hard to perform the attacks at a large scale, and 2) It targets the recommendation list of selected victim users only, thus it is not suitable if the attacker wants to promote an item indifferently to the general public. The shilling attack proposed in this paper does not suffer from these limitations.

%We note that Xing et al.~\cite{xing2013take} also briefly discussed fake co-visitation injection attacks. 
%However, they didn't systematically model the attacks or evaluate their effectiveness and feasibility at scale.  
% attack aims to attack per-profile recommendations. 
%Specifically, they pollute a targeted user's profile via CSRF. 
%Hard to scale because of relying on CSRF. 


 
\subsubsection{Privacy Attacks} Two attacks, i.e., \emph{item inference attacks} and \emph{attribute inference attacks}, were proposed to compromise user privacy in recommender systems.


\myparatight{Item inference attacks} Calandrino et al.~\cite{CalandrinoOakland11} proposed privacy attacks to infer the items that a target user has rated before, e.g., such items could be products that the target user purchased on Amazon, music the target user liked on Last.fm, and books the target user read on LibraryThing. The key intuition of their attacks is that a collaborative filtering recommender system makes recommendations based on users' past behavior. Therefore, the recommendations made by a recommender system include information about users' past behavior. Via tracking and analyzing the publicly available recommendations over time, an attacker could infer a target user's past behavior, e.g., the items the user rated. 


%Recommendation results are commonly generated by analyze a user's profile and thus may reflect the user's private information in an implicit way. Calandrino et al.~\cite{CalandrinoOakland11} proposed privacy attacks to infer such information (e.g., the products that the user purchased on eBay) by analyzing the recommendations made by the recommender system to users. Such recommendations are usually considered harmless to the user and thus are the publicly available. Specifically, in their privacy attacks, an attacker first obtains a partial profile of a user. For instance, on Amazon, some users will review some products that they purchased. Through collecting these publicly available reviews, the attacker can obtain a subset of products that the target user purchased. Then the attacker monitors the temporal changes of item-to-item recommendation lists of these products. If an item appears in the recommendation lists of a large number of products that are in the target user's partial profile, the attacker infers that the user purchased the item. The authors demonstrated that this privacy attack is feasible on various popular web services including Amazon, LibraryThing, Hunch, and Last.fm.



\myparatight{Attribute inference attacks} A user's rating behavior (e.g., rating scores to items, page likes on Facebook) is essentially statistically correlated to the user's attributes (e.g., gender, political view, sexual orientation, interests, and location). Therefore, an attacker could infer a user's private attributes based on its rating behavior via machine learning techniques, which capture the statistical correlations between rating behavior and attributes. Such attacks are called \emph{attribute inference attacks}~\cite{GongAttriInferSEC16} and have been demonstrated to be feasible by multiple studies~\cite{weinsberg2012blurme,kosinski2013private,Gong14,GongAttriInferSEC16,AttriInfer,gongTOPS18}. In particular, given a set of users whose rating behavior and attributes are known to an attacker, the attacker learns a machine learning classifier which takes a user's rating behavior as an input and predicts the user's attributes. Then, the attacker applies this classifier to infer attributes of the users who did not disclose their attributes. A notable example of real-world attribute inference attacks is that Cambridge Analytica leveraged Facebook users' rating behavior (e.g., page likes) to infer users' attributes, based on which targeted advertisements are delivered to users~\cite{Cambridge}. Jia and Gong~\cite{Jia18} recently proposed a practical defense against attribute inference attacks via adversarial machine learning. The key idea is to add carefully crafted noise to a user's rating behavior data such that the attacker's classifier is very likely to make incorrect predictions.  







==> macros.tex <==
%auto-ignore
% The name of this file is ``macros.tex''
%

%
% TEX defaults
%
%
% frame 6.5 * 9
\textwidth 6.5in
\textheight 9in

% left/right margins
\oddsidemargin 0pt
\evensidemargin 0pt
\marginparwidth 1in
\marginparsep 0pt

% top margin
\topmargin -25pt
\headheight 10pt
\headsep 30pt
% \topskip 0pt

% foot margin
%\footheight 0pt
\footskip 27pt


% macros for commonly used special fonts
\newcommand{\IE}{{\it i.e.,}\ }
\newcommand{\EG}{{\it e.g.,}\ }
% single/double spacing
%\newcommand{\SS}{\renewcommand{\baselinestretch}{1}\large\normalsize}
\newcommand{\DS}{\renewcommand{\baselinestretch}{1.6}\large\normalsize}
% reduce the space between lines
\newcommand{\Tight}{\renewcommand{\baselinestretch}{0.9}\large\normalsize}
\newcommand{\HalfTight}{\renewcommand{\baselinestretch}{0.95}\large\normalsize}
\newcommand{\MinorTight}{\renewcommand{\baselinestretch}{0.975}\large\normalsize}
% Page title (primarily for foils)
% (this was called \HH}
\newcommand{\PageTitle}[1]{{\newpage \begin{center}{\LARGE {\bf {#1}} } \end{center} } }

% remove spaces around section headers
%\newcommand{\Section}[1]{\vspace{-3ex}\section{#1}\vspace{-2ex}}
\newcommand{\Subsection}[1]{\vspace{-2ex}\subsection{#1}\vspace{-1ex}}
\newcommand{\Subsubsection}[1]{\vspace{-2ex}\subsubsection{#1}\vspace{-1ex}}

% go forward n lines (negative for backward move)
\newcommand{\VLine}[1]{\vspace{#1ex}}
% itemize and enumerate without spaces around/between items
\newenvironment{TightItem}{\vspace{-2ex}\begin{itemize}
  \setlength{\itemsep}{-0ex}}{\end{itemize}\vspace{-1ex}}
\newenvironment{TightEnum}{\vspace{-2ex}\begin{enumerate}
  \setlength{\itemsep}{-0ex}}{\end{enumerate}\vspace{-1ex}}
\newenvironment{TightDesc}{\vspace{-1ex}\begin{description}
  \setlength{\itemsep}{-0ex}}{\end{description}\vspace{-1ex}}
% set the page number (to the first argument)
\newcommand{\SetPageNo}[1]{\countdef\pageno=0 \pageno=#1}
% things to do
\newenvironment{Todo}{\begin{large}\begin{bf}********** things to do
    ********** \\}{\\ **********\end{bf}\end{large}}
% for discussion
\newenvironment{Discuss}{\begin{large}\begin{em}**********
    things to be discussed ********** \\}{\\ **********\end{em}\end{large}}
% set the paragraph identation and separation


% the foil environment
\newenvironment{Foil}{\begin{document}\begin{LARGE}\begin{sf}
    }{\end{sf}\end{LARGE}\end{document}}
    % NOTE: ``}'' must be in the 2nd line
% foil page title
\newcommand{\Title}[1]{\newpage \center{\huge {\sf #1}} \flushleft
    \vspace{1ex}}

% set the paragraph identation and separation
\parindent 0.2in
\setlength{\parskip}{1ex}

% set text width
\textwidth = 6.75in

% set the formula separation
\setlength{\topsep}{0in}

% set indentation for formulas:
% \setlength{\mathindent}{3ex}

% set left margin
\setlength{\oddsidemargin}{-.1in}




==> model.tex <==
%auto-ignore
\section{Long Short Term Memory Enhanced Spatio-Temporal Point Process}\label{sec:model}

Equation~(\ref{density}) shows that traditional TPP models depend conditionally on $H$, the time of historical events. Let $u$ and $l$ denote the user and location of interest, respectively (an event being $u$ check-in to $l$). As we discussed before, such historical events are scarce in check-in data due to the lack of repeated check-ins to the same location by a user. This causes difficulties in both training and predicting stage of TPP models. We propose to enrich the event sequences with \textit{Precedent Check-ins}, which are check-ins a user reported before check-in to $l$ on his/her trajectory. Figure~\ref{sequence} illustrates a normal sequence of events and the same sequence enriched with precedent check-ins.

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.40]{sequence.pdf}
\end{center}
\caption{Example of an enriched event sequence. }\label{sequence}
%\vspace{-7mm}
\end{figure}

Recall the previous example of visiting restaurants and shops. If a user check-ins to a restaurant, this behaviour shall decrease the user's intensity to visit another restaurant at the moment. But check-in to a shop may not effect the intensity to visit a nearby shop of the same type. Similarly, moving towards or away from a location shall cause the intensity to visit the location to fluctuate accordingly. These examples are only to demonstrate the possible influence of precedent check-ins on the intensity function. The actual dependency could be much more complex, for which we will have the LSTM-STPP model to discover from the check-in data.


\subsection{Feature Representation}

Before we feed an enriched event sequence to our model, each check-in in the sequence needs to be represented as a feature vector, which contains the information about the check-in in a structured manner. The feature vector for a check-in $c_i$ is denoted by $\boldsymbol{y_i}$, which consists of the following elements:

\begin{enumerate}[leftmargin=*]
\item Localized event time $t_i \in \mathbb{R}$. Time of the earliest check-in to the location is set to 0 and the rest times are set accordingly in the unit of hours or days.

\item Additional time-date information which indicates if the check-in occurred in a weekday or a weekend, and in what time period of the day (e.g., morning, afternoon, or midnight). This is because human demonstrates different check-in patterns in different time periods.

\item Euclidean distance of the check-in location to the location of interest $l$. The distance is computed using coordinates of the locations and normalized to the range of $[0,1]$, where $1$ indicates the distance is negligible, while $0$ means the distance is larger than a distance threshold denoted by $\theta_D$. 

\item Category of the check-in location, such as \textit{Restaurant, Hotel, Bar,} etc. We use a $x$-dimension value to represent the category information where $x$ is the total number of location categories. The $i$-th element is set to $1$ if the location belongs to the $i$-th category, otherwise $0$.

\item User overlapping with the location of interest $l$. Let $p$ denote the check-in location of $c_i$. We compute the proportion of users that have visited both $p$ and $l$ within a given time window. It reflects the inherent relevance of the two locations. The overlapping ratio is computed as follows:
\begin{align}
OR = C_{l,p}^v \Big/ \sqrt{C_l^v C_p^v},
\end{align}
where $C_{l,p}^v$ is the number of users who visited both $l$ and $p$ within a time window $v$. $C_l^v$ and $C_p^v$ are the number of visitors to $l$ and $p$ within the time window, respectively.

\item Previous check-in by friends, which reflects the social aspect of check-in behaviors. We calculate the minimal time interval from $t_i$ to a check-in to the location of interest by a friend of the user. The value is normalized such that $1$ indicates a friend just check-in to the location, while $0$ means the minimal time interval is larger than a threshold denoted by $\theta_T$.

\end{enumerate}

Each vector is also associated with a Boolean value indicating if it is an event or a precedent check-in. Unfortunately, not all the above information are always available on LBSNs. e.g., some LBSNs hide user's social connections, or do not provide location categories. In such cases the unavailable features are ignored in generating the vector. Therefore, the total dimension of the feature vector may vary depending on the specific data source. Comparing with $\boldsymbol{y_i}$, the user feature vector $\boldsymbol{p_u}$ is simpler. It contains two elements. 

The first element is the user's preference to the location of interest $l$. We incorporate both explicit and implicit preference. Explicit preference is the user's rating for $l$, which is usually not directly available for every location, but can be estimated using techniques such as matrix factorization~\cite{koren2009matrix}. As for implicit preference, we calculate the user's check-in frequency to $l$, i.e., the total number of check-ins to $l$ on the user's trajectory, divided by the length (time between the first and the last check-in) of the trajectory.

The second element is the user's homebase, i.e., the center and range of the user's daily movements. The explicit homebase are usually unknown. Here we use the method introduced in~\cite{yang2016spatio} to estimate a user's homebase using the distribution of his historical check-ins. We then use the normalized distance from the estimated homebase to the location of interest as the feature value.


\subsection{Model Architecture}

Figure~\ref{RNN} gives a high-level illustration of the proposed model, which consists of an input layer, an output layer, several hidden layers, and inner weight matrices that store weights on the edges. 

\begin{figure}[htbp]
\begin{center}
\includegraphics[scale=0.55]{RNN.pdf}
\end{center}
\caption{LSTM-STPP model architecture.}\label{RNN}
%\vspace{-7mm}
\end{figure}

The input to the model is a sequence of events enriched with precedent check-ins, denoted by $\{ c_1, c_2, ..., c_n \}$ where $c_i$ $(1 \leq i \leq n-1)$ can be either an event or a precedent check-in. Using these check-ins, we want to predict the next event time after $C_n$. When feed into the model, a check-in $c_i$ is represented by a feature vector $\boldsymbol{y_i}$. The model then iterates through the input sequence in $n$ steps, and updates its status at each step.

We now discuss how to update the internal status of the neural network. The internal status of the model at the $i$-th step can be represented as a vector $\boldsymbol{h_i}$. In each step, the vector which is updated by several hidden neural network layers according to the previous network status and current inputs. The location information of check-ins is incorporated into the status vector during this updating process, which we illustrate in Figure~\ref{}.

The first step of status updating is to discard, or ``forget" irrelevant information from historical events. This is implemented by the forget gate layer $\boldsymbol{ F_t }$, which is computed as follows in our model:
\begin{align}
\boldsymbol{ F_t } = 	\begin{cases} 
		g( \boldsymbol{ M_F } *[ \boldsymbol{ h_{i-1}, Y_i }  ] + b_F), & \text{if } c_i \text{is an event} \\
		1 & \text{otherwise} 
		\end{cases}
\end{align}
Here, $\boldsymbol{ M_f }$ is the weight matrix of the forget gate layer, $b_F$ is a constant, and $g(\cdot)$ is an activation function, for which we choose the sigmoid function $g(x) = exp(1/1+e^{-x})$. $[ \cdot, \cdot]$ denotes the concatenation of two vectors. And finally, $\boldsymbol{Y_i}$ is the accumulated check-in information from successive check-ins occurred in a certain time window $w$, which is defined as follows:
\begin{align}
\boldsymbol{ Y_i } = \sum_{(t_i - t_j < w)} \boldsymbol{ M_{t_i - t_j} * y_j }
\end{align}
where the condition $t_i - t_j < w$ defines a time window that includes all the precedent check-ins and events within $w$ from the time of $c_i$ (including $c_i$). The time window $w$ can be further partitioned into several intervals, and $M_{t_i - t_j}$ is a transition matrix specifically for the internal that covers $t_i - t_j$.  This term is meant to capture the influence of recent precedent check-ins in different time windows that may lead to the current event.

Then, the model decides which new information shall be stored, this is implemented with two separated neural network layers, the input gate layer $ \boldsymbol{I_i}
$ and the candidate cell status layer $\boldsymbol{\tilde{S}_i}$. We have the following updating functions:
\begin{align}
\boldsymbol{I_i} = \begin{cases}
	   g( \boldsymbol{ M_I } * [ \boldsymbol{ h_{i-1}, Y_i }  ] + b_I ), & \text{if } c_i \text{is an event} \\
	   g( \boldsymbol{ M_I'} * [ \boldsymbol{ h_{i-1}, y_i } ] + b_I' ), & \text{otherwise} 
	   \end{cases}   
\end{align}

\begin{align}
\boldsymbol{\tilde{S}_i} = \begin{cases}
	   			h( \boldsymbol{ M_S } [ \boldsymbol{ h_{i-1}, Y_i}  ] + b_S), & \text{if } c_i \text{is an event} \\
	  			h( \boldsymbol{ M_S' } [ \boldsymbol{ h_{i-1}, y_i} ] + b_S'), & \text{otherwise} 
	   		   \end{cases}
\end{align}
In the above equations, $\boldsymbol{M_I, M_I', M_S, M_S'}$ are weight matrices and $b_I,b_I',b_S,b_S'$ are constant parameters. $h$ is another activation function which we use $tanh(\cdot)$ since we want the output value to be in the range of $[-1,1]$.

The next step is to update the cell status, denoted by $\boldsymbol{S_i}$. It is updated by ``forget" the information marked by the forget gate layer while ``remember" new information provided by the input gate and candidate status layer:
\begin{align}
\boldsymbol{S_i} = \boldsymbol{ F_t S_{i-1}} + \boldsymbol{ I_i \tilde{S}_i}
\end{align}
After the updating, the cell status now records the information that should be passed to the next step. And finally, we can update the vector representation of the  internal network status:
\begin{align}
\boldsymbol{h_i} = \begin{cases}
	   g( \boldsymbol{ M_H } [ \boldsymbol{ h_{i-1}, Y_i}  ] + b_H) h(\boldsymbol{S_i}), & \text{if } c_i \text{is an event} \\
	   g( \boldsymbol{ M_H' } [ \boldsymbol{ h_{i-1}, y_i} ] + b_H') h(\boldsymbol{S_i}), & \text{otherwise}
	  \end{cases}   
\end{align}
Note that both $\boldsymbol{S_i}$ and $\boldsymbol{h_i}$ are passed to the next step of the model, thus an recurrent status update is implemented.

Intuitively, the status vector $\boldsymbol{h_i}$ can be seen as a latent representation of knowledge learned from all previous check-ins by the model. We can now compute the conditional density function of next event time using $\boldsymbol{h_i}$ as follows:
\begin{align}
\lambda(t) = exp \Big( \boldsymbol{W}^T \boldsymbol{ h_i} + \beta_t (t-t_i) + \beta_d D + \boldsymbol{B}^T \boldsymbol{p_u} + b \Big)
\end{align}
The computation involves several factors: $\boldsymbol{W}^T \boldsymbol{ h_i}$ computes the influence of previous check-ins, $\beta_t (t-t_i)$ and $\beta_d d$ represent current temporal and spatial impact, respectively, and $D$ is the Euclidean distance between current location and the location of interest. The vector $\boldsymbol{p_u}$ represents information of the user, which allows the function to be personalized for a given user $u$. Finally, $b$ is a constant base intensity for the location. Note that the exponential function guarantees the intensity is positive.

The intensity function is then used to predict the time interval between current check-in $c_i$ and the next event $c_j$:
\begin{align}
\hat{I}_{i,j} = \hat{t}_{j} - t_i,
\end{align}
where $\hat{t}_{j}$ is estimated using Equation~(\ref{expect}). The predicted value $\hat{I}_{i,j}$ is the only output of the model at each step. 

Note that the LSTM-STPP model may generate multiple predictions for the time of the same event. This is because if an event has precedent check-ins, each of the check-ins will generate an output but they have the same next-event. In this case, we will use the output of the most recent precedent check-in as the final prediction for the event time. There are two reasons behind this: First, temporally close check-ins are usually more relevant to each other. Second: The output of the most recent precedent check-in is supposed to incorporate information of all the precedent check-ins and historical events, thus shall contain more complete information. If an event has no direct precedent check-ins, i.e., it is preceded by another event with no other check-in in between, then the event will have a single predicted time. This design guarantees that a valid prediction can be made even for users who have never visited the location of interest. In that case, all his/her check-ins will be treated as precedent check-ins, and no event is included in the sequence.

% Multiple predictions for the same time point...

\subsection{Model Training}

For a given location of interest, the training dataset is a collection of historical user trajectories. Each trajectory contains at least one check-in to the location as ground truth. We use the classic Back Propagation Through Time~\cite{rumelhart1988learning} for LSTM networks to train the proposed RSTPP model. We use the cycle unrolling technique and unroll the recurrent neural network by $s$ steps. The model parameters are shared among the unrolled copies of the neural network. Similarly, the training sequences are also partitioned into batches of subsequence which contains at least $s$ consecutive check-ins. The loss function we used is the negative log-likelihood of observing the training instances (given in Equation~\ref{MLE}). In each iteration of the training process, output of the model is feed into the loss function and its parameters are updated accordingly in the back propagation stage using stochastic gradient descent until achieve convergence.
